MODULI: Unlocking Preference Generalization via Diffusion Models for Offline Multi-Objective Reinforcement Learning

Multi-objective Reinforcement Learning (MORL) seeks to develop policies that simultaneously optimize multiple conflicting objectives, but it requires extensive online interactions. Offline MORL provides a promising solution by training on pre-collected datasets to generalize to any preference upon deployment. However, real-world offline datasets are often conservatively and narrowly distributed, failing to comprehensively cover preferences, leading to the emergence of out-of-distribution (OOD) preference areas. Existing offline MORL algorithms exhibit poor generalization to OOD preferences, resulting in policies that do not align with preferences. Leveraging the excellent expressive and generalization capabilities of diffusion models, we propose MODULI (Multi-objective Diffusion Planner with Sliding Guidance), which employs a preference-conditioned diffusion model as a planner to generate trajectories that align with various preferences and derive action for decision-making. To achieve accurate generation, MODULI introduces two return normalization methods under diverse preferences for refining guidance. To further enhance generalization to OOD preferences, MODULI proposes a novel sliding guidance mechanism, which involves training an additional slider adapter to capture the direction of preference changes. Incorporating the slider, it transitions from in-distribution (ID) preferences to generating OOD preferences, patching, and extending the incomplete Pareto front. Extensive experiments on the D4MORL benchmark demonstrate that our algorithm outperforms state-of-the-art Offline MORL baselines, exhibiting excellent generalization to OOD preferences.

==> tables/compare_guidance_full.tex <==
\begin{table*}[htb]
  \caption{compare of different guide methods on \texttt{Shattered} datasets. The following MODULIs all contain sliders.}
  \label{sample-table}
  \centering
  \begin{tabular}{p{0.03\textwidth}p{0.1\textwidth}p{0.12\textwidth}||p{0.1\textwidth}p{0.1\textwidth}p{0.1\textwidth}}
    \toprule
    ~ & \textbf{Env} & metrics & \textbf{MODULI} & \textbf{CFG+CG} & \textbf{CG} \\
    \midrule
    \multirow{20}*{\rotatebox{90}{Amateur}} & \multirow{3}*{Ant}         & HV ($\times 10^{6}$) $\uparrow$ & \textbf{6.04±.01} & 6.00±.02 & 5.79±.00 \\
    ~                                       & ~                          & RM ($\times 10^{3}$) $\downarrow$ & \textbf{0.09±.01} & 0.11±.01 & 0.87±.02 \\
    ~                                       & ~                          & SP ($\times 10^{4}$) $\downarrow$ & 0.63±.23 & 0.52±.07 & 0.53±.11 \\
    \cmidrule{2-6}
    ~                                       & \multirow{3}*{HalfCheetah} & HV ($\times 10^{6}$) $\uparrow$ & \textbf{5.75±.00} & 5.74±.00 & 5.68±.03 \\
    ~                                       & ~                          & RM ($\times 10^{3}$) $\downarrow$ & \textbf{0.07±.00} & 0.08±.00 & 0.63±.02 \\
    ~                                       & ~                          & SP ($\times 10^{4}$) $\downarrow$ & 0.14±.01 & 0.11±.01 & 0.22±.08 \\
    \cmidrule{2-6}
    ~                                       & \multirow{3}*{Hopper}      & HV ($\times 10^{7}$) $\uparrow$ & \textbf{2.01±.01} & 1.91±.01 & 1.95±.01 \\
    ~                                       & ~                          & RM ($\times 10^{3}$) $\downarrow$ & \textbf{0.49±.15} & 0.66±.08 & 0.52±.10 \\
    ~                                       & ~                          & SP ($\times 10^{5}$) $\downarrow$ & 0.15±.04 & 0.37±.13 & 0.17±.02 \\
    \cmidrule{2-6}
    ~                                       & \multirow{3}*{Swimmer}     & HV ($\times 10^{4}$) $\uparrow$ & \textbf{3.17±.00} & 3.13±.01 & 3.01±.00 \\
    ~                                       & ~                          & RM ($\times 10^{2}$) $\downarrow$ & 0.29±.00 & 0.38±.01 & \textbf{0.28±.00} \\
    ~                                       & ~                          & SP ($\times 10^{0}$) $\downarrow$ & 9.65±.70 & 24.45±2.25 & 8.37±1.46 \\
    \cmidrule{2-6}
    ~                                       & \multirow{3}*{Walker2d}    & HV ($\times 10^{6}$) $\uparrow$ & \textbf{5.02±.00} & 4.96±.00 & 4.93±.00 \\
    ~                                       & ~                          & RM ($\times 10^{3}$) $\downarrow$ & \textbf{0.37±.01} & 0.69±.03 & 0.55±.02 \\
    ~                                       & ~                          & SP ($\times 10^{4}$) $\downarrow$ & 0.30±.03 & 0.55±.03 & 0.80±.01 \\
    \cmidrule{2-6}
    ~                                       & \multirow{3}*{Hopper-3obj} & HV ($\times 10^{10}$) $\uparrow$ & \textbf{3.02±.03} & 2.78±.09 & 2.59±.14 \\
    ~                                       & ~                          & RM ($\times 10^{3}$) $\downarrow$ & \textbf{1.01±.04} & 1.70±.05 & 1.75±.07 \\
    ~                                       & ~                          & SP ($\times 10^{5}$) $\downarrow$ & 0.10±.01 & 0.09±.01 & 0.07±.03 \\
    \cmidrule[\heavyrulewidth]{1-6}
    \multirow{20}*{\rotatebox{90}{Expert}}  & \multirow{3}*{Ant}         & HV ($\times 10^{6}$) $\uparrow$ & \textbf{6.39±.01} & 6.36±.03 & 6.23±.03 \\
    ~                                       & ~                          & RM ($\times 10^{3}$) $\downarrow$ & \textbf{0.14±.01} & \textbf{0.14±.00} & 0.46±.02 \\
    ~                                       & ~                          & SP ($\times 10^{4}$) $\downarrow$ & 0.53±.13 & 0.52±.13 & 0.52±.16 \\
    \cmidrule{2-6}
    ~                                       & \multirow{3}*{HalfCheetah} & HV ($\times 10^{6}$) $\uparrow$ & \textbf{5.78±.00} & \textbf{5.78±.00} & 5.69±.01 \\
    ~                                       & ~                          & RM ($\times 10^{3}$) $\downarrow$ & \textbf{0.07±.00} & \textbf{0.07±.00} & 0.37±.02 \\
    ~                                       & ~                          & SP ($\times 10^{4}$) $\downarrow$ & 0.11±.02 & 0.10±.02 & 0.47±.03 \\
    \cmidrule{2-6}
    ~                                       & \multirow{3}*{Hopper}      & HV ($\times 10^{7}$) $\uparrow$ & \textbf{2.07±.00} & \textbf{2.07±.01} & 1.95±.01 \\
    ~                                       & ~                          & RM ($\times 10^{3}$) $\downarrow$ & \textbf{0.22±.06} & 0.23±.03 & 0.81±.19 \\
    ~                                       & ~                          & SP ($\times 10^{5}$) $\downarrow$ & 0.11±.01 & 0.09±.01 & 0.09±.01 \\
    \cmidrule{2-6}
    ~                                       & \multirow{3}*{Swimmer}     & HV ($\times 10^{4}$) $\uparrow$ & \textbf{3.24±.00} & \textbf{3.24±.00} & 3.19±.01 \\
    ~                                       & ~                          & RM ($\times 10^{2}$) $\downarrow$ & 0.06±.00 & \textbf{0.04±.00} & 0.29±.02 \\
    ~                                       & ~                          & SP ($\times 10^{0}$) $\downarrow$ & 5.79±.43 & 6.78±1.26 & 23.28±3.56 \\
    \cmidrule{2-6}
    ~                                       & \multirow{3}*{Walker2d}    & HV ($\times 10^{6}$) $\uparrow$ & \textbf{5.20±.00} & 5.19±.00 & 5.01±.06 \\
    ~                                       & ~                          & RM ($\times 10^{3}$) $\downarrow$ & \textbf{0.15±.01} & 0.17±.00 & 0.73±.04 \\
    ~                                       & ~                          & SP ($\times 10^{4}$) $\downarrow$ & 0.12±.01 & 0.12±.02 & 1.27±.32 \\
    \cmidrule{2-6}
    ~                                       & \multirow{3}*{Hopper-3obj} & HV ($\times 10^{10}$) $\uparrow$ & \textbf{3.43±.02} & 3.39±.02 & 2.30±.08 \\
    ~                                       & ~                          & RM ($\times 10^{3}$) $\downarrow$ & \textbf{1.28±.03} & 1.66±.01 & 2.45±.10 \\
    ~                                       & ~                          & SP ($\times 10^{5}$) $\downarrow$ & 0.10±.01 & 0.12±.01 & 0.10±.01 \\

    \bottomrule
  \end{tabular}
\end{table*}



==> tables/compare_guidance_partial.tex <==
\begin{table*}[htb]
  \caption{compare of different guide methods on \texttt{Shattered} and \texttt{Narrow} datasets.}
  \label{sample-table}
  \centering
  \begin{tabular}{p{0.03\textwidth}p{0.1\textwidth}p{0.11\textwidth}||p{0.1\textwidth}p{0.1\textwidth}p{0.1\textwidth}}
    \toprule
    ~ & \textbf{Env} & metrics & \textbf{MODULI w slider} & \textbf{CFG+CG} & \textbf{CG} \\
    \midrule
    \multirow{6}*{\rotatebox{90}{Shattered}} & \multirow{3}*{Hopper}      & HV ($\times 10^{7}$) & \textbf{2.01±.00} & 1.91±.01 & 1.95±.01 \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & \textbf{4.00±.04} & 3.86±.00 & 3.97±.03 \\
    ~                                       & ~                          & SP ($\times 10^{5}$) & 0.19±.01 & 0.37±.13 & 0.17±.02 \\
    \cmidrule{2-6}
    ~                                       & \multirow{3}*{Swimmer}     & HV ($\times 10^{4}$) & \textbf{3.18±.00} & 3.13±.01 & 3.01±.00 \\
    ~                                       & ~                          & WR ($\times 10^{2}$) & \textbf{1.65±.02} & 1.62±.01 & 1.51±.01 \\
    ~                                       & ~                          & SP ($\times 10^{0}$) & 15.71±.61 & 24.45±2.25 & 8.37±1.46 \\
    \cmidrule[\heavyrulewidth]{1-6}
    \multirow{6}*{\rotatebox{90}{Narrow}}  & \multirow{3}*{Hopper}      & HV ($\times 10^{7}$) & \textbf{2.01±.01} & 1.91±.01 & 1.95±.01 \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & \textbf{3.99±.01} & 3.86±.00 & 3.97±.03 \\
    ~                                       & ~                          & SP ($\times 10^{5}$) & 0.18±.02 & 0.37±.13 & 0.17±.02 \\
    \cmidrule{2-6}
    ~                                       & \multirow{3}*{Swimmer}     & HV ($\times 10^{4}$) & \textbf{3.16±.00} & 3.13±.01 & 3.01±.00 \\
    ~                                       & ~                          & WR ($\times 10^{2}$) & \textbf{1.63±.01} & 1.62±.01 & 1.51±.01 \\
    ~                                       & ~                          & SP ($\times 10^{0}$) & 10.54±1.45 & 24.45±2.25 & 8.37±1.46 \\
    \bottomrule
  \end{tabular}
\end{table*}

==> tables/compare_newrvs.tex <==
\begin{table*}[htb]
  \caption{compare of rvs preformance and our reproduced one}
  \label{sample-table}
  \centering
  \begin{tabular}{p{0.03\textwidth}p{0.1\textwidth}p{0.1\textwidth}||p{0.05\textwidth}|p{0.1\textwidth}p{0.1\textwidth}p{0.1\textwidth}|p{0.15\textwidth}p{0.1\textwidth}}
    \toprule
    ~ & \textbf{Env} & metrics & \textbf{B} & \textbf{MODT(P)} & \textbf{MORvS(P)} & \textbf{BC(P)} & \textbf{MORvS(P)(NEW)} & \textbf{MODULI} \\
    \midrule
    \multirow{15}*{\rotatebox{90}{Amateur}} & \multirow{2}*{Ant}         & HV ($\times 10^{6}$) & 5.61 & 5.92±.04 & 6.07±.02 & 4.37±.06 & 6.05±.01 & \textbf{6.08±.03} \\
    ~                                       & ~                          & SP ($\times 10^{4}$) & - & 8.72±.77 & 5.24±.52 & 25.90±16.40 & 0.72±.13 & \textbf{0.53±.05} \\
    \cmidrule{2-9}
    ~                                       & \multirow{2}*{HalfCheetah} & HV ($\times 10^{6}$) & 5.68 & 5.69±.01 & \textbf{5.77±.00} & 5.46±.02 & 5.74±.00 & 5.76±.00 \\
    ~                                       & ~                          & SP ($\times 10^{4}$) & - & 1.16±.42 & 0.57±.09 & 2.22±.91 & 0.10±.01 & \textbf{0.07±.02} \\
    \cmidrule{2-9}
    ~                                       & \multirow{2}*{Hopper}      & HV ($\times 10^{7}$) & 1.97 & 1.81±.05 & 1.76±.03 & 1.35±.03 & 1.83±.01 & \textbf{2.01±.01} \\
    ~                                       & ~                          & SP ($\times 10^{5}$) & - & 1.61±.29 & 3.50±1.54 & 2.42±1.08 & \textbf{0.10±.01} & \textbf{0.10±.01} \\
    \cmidrule{2-9}
    ~                                       & \multirow{2}*{Swimmer}     & HV ($\times 10^{4}$) & 2.11 & 1.67±.22 & 2.79±.03 & 2.82±.04 & 2.77±.00 & \textbf{3.20±.00} \\
    ~                                       & ~                          & SP ($\times 10^{0}$) & - & 2.87±1.32 & 1.03±.20 & 5.05±1.82 & \textbf{0.98±.02} & 9.50±.59 \\
    \cmidrule{2-9}
    ~                                       & \multirow{2}*{Walker2d}    & HV ($\times 10^{6}$) & 4.99 & 3.10±.34 & 4.98±.01 & 3.42±.42 & 4.99±.00 & \textbf{5.06±.00} \\
    ~                                       & ~                          & SP ($\times 10^{4}$) & - & 164.20±13.50 & 1.94±.06 & 53.10±34.60 & \textbf{0.17±.02} & 0.25±.03 \\
    \cmidrule{2-9}
    ~                                       & \multirow{2}*{Hopper-3obj} & HV ($\times 10^{10}$) & 3.09 & 1.04±.16 & 2.77±.24 & 2.42±.18 & 2.84±.04 & \textbf{3.33±.06} \\
    ~                                       & ~                          & SP ($\times 10^{5}$) & - & 10.23±2.78 & 1.03±.11 & 0.87±.29 & 0.11±.01 & \textbf{0.10±.00} \\
    \cmidrule[\heavyrulewidth]{1-9}
    \multirow{15}*{\rotatebox{90}{Expert}}  & \multirow{2}*{Ant}         & HV ($\times 10^{6}$) & 6.32 & 6.21±.01 & \textbf{6.41±.01} & 4.88±.17 & 6.36±.02 & 6.39±.02 \\
    ~                                       & ~                          & SP ($\times 10^{4}$) & - & 8.26±2.22 & 6.50±.81 & 46.20±16.40 & 0.87±.19 & \textbf{0.79±.12} \\
    \cmidrule{2-9}
    ~                                       & \multirow{2}*{HalfCheetah} & HV ($\times 10^{6}$) & 5.79 & 5.73±.00 & 5.78±.00 & 5.54±.05 & 5.74±.01 & \textbf{5.79±.00} \\
    ~                                       & ~                          & SP ($\times 10^{4}$) & - & 1.24±.23 & 0.67±.05 & 1.78±.39 & 0.16±.01 & \textbf{0.07±.00} \\
    \cmidrule{2-9}
    ~                                       & \multirow{2}*{Hopper}      & HV ($\times 10^{7}$) & 2.09 & 2.00±.02 & 2.02±.02 & 1.23±.10 & 1.98±.05 & \textbf{2.09±.01} \\
    ~                                       & ~                          & SP ($\times 10^{5}$) & - & 16.30±10.60 & 3.03±.36 & 52.50±4.88 & 0.26±.13 & \textbf{0.09±.01} \\
    \cmidrule{2-9}
    ~                                       & \multirow{2}*{Swimmer}     & HV ($\times 10^{4}$) & 3.25 & 3.15±.02 & 3.24±.00 & 3.21±.00 & \textbf{3.25±.00} & 3.24±.00 \\
    ~                                       & ~                          & SP ($\times 10^{0}$) & - & 15.00±7.49 & \textbf{4.39±.07} & 4.50±.39 & 4.51±.42 & 4.43±.38 \\
    \cmidrule{2-9}
    ~                                       & \multirow{2}*{Walker2d}    & HV ($\times 10^{6}$) & 5.21 & 4.89±.05 & 5.14±.01 & 3.74±.11 & 5.14±.01 & \textbf{5.20±.00} \\
    ~                                       & ~                          & SP ($\times 10^{4}$) & - & 0.99±.44 & 3.22±.73 & 75.60±52.30 & 0.30±.03 & \textbf{0.11±.01} \\
    \cmidrule{2-9}
    ~                                       & \multirow{2}*{Hopper-3obj} & HV ($\times 10^{10}$) & 3.73 & 3.38±.05 & 3.42±.10 & 2.29±.07 & 3.28±.07 & \textbf{3.57±.02} \\
    ~                                       & ~                          & SP ($\times 10^{5}$) & - & 1.40±.44 & 2.72±1.93 & 0.72±.09 & \textbf{0.06±.00} & 0.07±.00 \\

    \bottomrule
  \end{tabular}
\end{table*}


==> tables/compare_norm_new_full.tex <==
\begin{table*}[htb]
  \caption{Compare of different normalization methods on \texttt{Complete} datasets.}
  \label{sample-table}
  \centering
  \begin{tabular}{p{0.03\textwidth}p{0.1\textwidth}p{0.12\textwidth}||p{0.1\textwidth}p{0.1\textwidth}p{0.1\textwidth}}
    \toprule
    ~ & \textbf{Env} & metrics & \textbf{Neighborhood Preference Normalization} & \textbf{Preference Predicted Normalization} & \textbf{Global Normalization} \\
    \midrule
    \multirow{20}*{\rotatebox{90}{Amateur}} & \multirow{3}*{Ant}         & HV ($\times 10^{6}$) $\uparrow$ & \textbf{6.12±.03} & 6.01±.02 & 6.07±.03 \\
    ~                                       & ~                          & RM ($\times 10^{3}$) $\downarrow$ & \textbf{0.09±.00} & 0.10±.01 & 0.29±.00 \\
    ~                                       & ~                          & SP ($\times 10^{4}$) $\downarrow$ & 0.92±.15 & 0.80±.12 & 0.52±.12 \\
    \cmidrule{2-6}
    ~                                       & \multirow{3}*{HalfCheetah} & HV ($\times 10^{6}$) $\uparrow$ & 5.76±.00 & \textbf{5.77±.00} & 5.50±.02 \\
    ~                                       & ~                          & RM ($\times 10^{3}$) $\downarrow$ & 0.11±.00 & \textbf{0.03±.00} & 0.34±.00 \\
    ~                                       & ~                          & SP ($\times 10^{4}$) $\downarrow$ & 0.10±.00 & 0.07±.00 & 0.03±.00 \\
    \cmidrule{2-6}
    ~                                       & \multirow{3}*{Hopper}      & HV ($\times 10^{7}$) $\uparrow$ & \textbf{1.98±.02} & 1.94±.01 & 1.58±.02 \\
    ~                                       & ~                          & RM ($\times 10^{3}$) $\downarrow$ & 0.50±.14 & \textbf{0.34±.03} & 0.95±.03 \\
    ~                                       & ~                          & SP ($\times 10^{5}$) $\downarrow$ & 0.21±.06 & 0.24±.06 & 0.12±.03 \\
    \cmidrule{2-6}
    ~                                       & \multirow{3}*{Swimmer}     & HV ($\times 10^{4}$) $\uparrow$ & 3.14±.00 & \textbf{3.17±.00} & 2.54±.00 \\
    ~                                       & ~                          & RM ($\times 10^{2}$) $\downarrow$ & 0.55±.00 & \textbf{0.52±.00} & 0.81±.00 \\
    ~                                       & ~                          & SP ($\times 10^{0}$) $\downarrow$ & 9.29±.46 & 8.18±.48 & 2.82±.06 \\
    \cmidrule{2-6}
    ~                                       & \multirow{3}*{Walker2d}    & HV ($\times 10^{6}$) $\uparrow$ & \textbf{5.03±.00} & 4.94±.00 & 4.02±.01 \\
    ~                                       & ~                          & RM ($\times 10^{3}$) $\downarrow$ & 0.51±.05 & \textbf{0.23±.01} & 1.75±.00 \\
    ~                                       & ~                          & SP ($\times 10^{4}$) $\downarrow$ & 0.20±.01 & 0.31±.01 & 0.04±.01 \\
    \cmidrule{2-6}
    ~                                       & \multirow{3}*{Hopper-3obj} & HV ($\times 10^{10}$) $\uparrow$ & \textbf{3.33±.06} & 0.00±.00 & 2.22±.02 \\
    ~                                       & ~                          & RM ($\times 10^{3}$) $\downarrow$ & \textbf{1.15±.02} & 3.65±.00 & 2.30±.02 \\
    ~                                       & ~                          & SP ($\times 10^{5}$) $\downarrow$ & 0.10±.00 & 0.00±.00 & 0.22±.05 \\
    \cmidrule[\heavyrulewidth]{1-6}
    \multirow{20}*{\rotatebox{90}{Expert}}  & \multirow{3}*{Ant}         & HV ($\times 10^{6}$) $\uparrow$ & 6.35±.02 & 6.36±.01 & \textbf{6.38±.00} \\
    ~                                       & ~                          & RM ($\times 10^{3}$) $\downarrow$ & \textbf{0.14±.00} & 0.15±.01 & 0.24±.00 \\
    ~                                       & ~                          & SP ($\times 10^{4}$) $\downarrow$ & 0.62±.11 & 0.75±.11 & 0.99±.10 \\
    \cmidrule{2-6}
    ~                                       & \multirow{3}*{HalfCheetah} & HV ($\times 10^{6}$) $\uparrow$ & \textbf{5.79±.00} & \textbf{5.79±.00} & 5.57±.04 \\
    ~                                       & ~                          & RM ($\times 10^{3}$) $\downarrow$ & \textbf{0.03±.00} & 0.04±.00 & 0.30±.00 \\
    ~                                       & ~                          & SP ($\times 10^{4}$) $\downarrow$ & 0.06±.01 & 0.05±.01 & 0.02±.00 \\
    \cmidrule{2-6}
    ~                                       & \multirow{3}*{Hopper}      & HV ($\times 10^{7}$) $\uparrow$ & \textbf{2.07±.00} & \textbf{2.07±.01} & 1.48±.02 \\
    ~                                       & ~                          & RM ($\times 10^{3}$) $\downarrow$ & \textbf{0.28±.10} & 0.38±.05 & 3.94±.01 \\
    ~                                       & ~                          & SP ($\times 10^{5}$) $\downarrow$ & 0.14±.04 & 0.12±.02 & 2.69±1.97 \\
    \cmidrule{2-6}
    ~                                       & \multirow{3}*{Swimmer}     & HV ($\times 10^{4}$) $\uparrow$ & 3.24±.00 & \textbf{3.25±.00} & 2.62±.02 \\
    ~                                       & ~                          & RM ($\times 10^{2}$) $\downarrow$ & \textbf{0.08±.00} & 0.09±.00 & 1.64±.00 \\
    ~                                       & ~                          & SP ($\times 10^{0}$) $\downarrow$ & 5.86±.89 & 7.14±.55 & 20.81±25.36 \\
    \cmidrule{2-6}
    ~                                       & \multirow{3}*{Walker2d}    & HV ($\times 10^{6}$) $\uparrow$ & \textbf{5.20±.00} & 5.18±.00 & 2.70±.04 \\
    ~                                       & ~                          & RM ($\times 10^{3}$) $\downarrow$ & \textbf{0.02±.00} & 0.15±.02 & 2.33±.00 \\
    ~                                       & ~                          & SP ($\times 10^{4}$) $\downarrow$ & 0.11±.01 & 0.17±.01 & 5.11±6.88 \\
    \cmidrule{2-6}
    ~                                       & \multirow{3}*{Hopper-3obj} & HV ($\times 10^{10}$) $\uparrow$ & \textbf{3.57±.02} & 2.99±.04 & 0.53±.06 \\
    ~                                       & ~                          & RM ($\times 10^{3}$) $\downarrow$ & \textbf{1.32±.03} & 2.89±.01 & 3.82±.01 \\
    ~                                       & ~                          & SP ($\times 10^{5}$) $\downarrow$ & 0.07±.00 & 0.20±.03 & 1.12±.16 \\

    \bottomrule
  \end{tabular}
\end{table*}

==> tables/compare_norm_partial.tex <==
\begin{table*}[htb]
  \caption{HV}
  \label{sample-table}
  \centering
  \begin{tabular}{p{0.03\textwidth}p{0.1\textwidth}p{0.1\textwidth}||p{0.1\textwidth}p{0.1\textwidth}p{0.1\textwidth}}
    \toprule
    ~ & \textbf{Env} & metrics & \textbf{MODULI} & \textbf{MODULI w/o neighborhood normalization} & \textbf{MODULI global normalization} \\
    \midrule
    \multirow{15}*{\rotatebox{90}{Amateur}} & \multirow{2}*{Ant}         & HV ($\times 10^{6}$) & \textbf{6.12±.03} & 6.01±.02 & 6.09±.01 \\
    ~                                       & ~                          & SP ($\times 10^{4}$) & 0.92±.15 & 0.80±.12 & \textbf{0.55±.05} \\
    \cmidrule{2-6}
    ~                                       & \multirow{2}*{HalfCheetah} & HV ($\times 10^{6}$) & 5.76±.00 & \textbf{5.77±.00} & 5.73±.00 \\
    ~                                       & ~                          & SP ($\times 10^{4}$) & 0.10±.00 & 0.07±.00 & \textbf{0.04±.01} \\
    \cmidrule{2-6}
    ~                                       & \multirow{2}*{Hopper}      & HV ($\times 10^{7}$) & \textbf{1.98±.02} & 1.94±.01 & 0.01±.01 \\
    ~                                       & ~                          & SP ($\times 10^{5}$) & \textbf{0.21±.06} & 0.24±.06 & 0.68±.57 \\
    \cmidrule{2-6}
    ~                                       & \multirow{2}*{Swimmer}     & HV ($\times 10^{4}$) & 3.14±.00 & \textbf{3.17±.00} & 3.07±.00 \\
    ~                                       & ~                          & SP ($\times 10^{0}$) & 9.29±.46 & 8.18±.48 & \textbf{5.14±.73} \\
    \cmidrule{2-6}
    ~                                       & \multirow{2}*{Walker2d}    & HV ($\times 10^{6}$) & \textbf{5.03±.00} & 4.94±.00 & 4.64±.02 \\
    ~                                       & ~                          & SP ($\times 10^{4}$) & \textbf{0.20±.01} & 0.31±.01 & 0.75±.16 \\
    \cmidrule{2-6}
    ~                                       & \multirow{2}*{Hopper-3obj} & HV ($\times 10^{10}$) & \textbf{3.33±.06} & 0.00±.00 & 2.56±.06 \\
    ~                                       & ~                          & SP ($\times 10^{5}$) & \textbf{0.10±.00} & 0.00±.00 & 0.40±.12 \\
    \bottomrule
  \end{tabular}
\end{table*}

==> tables/main_results.tex <==
\begin{table*}[htb]
  \small
  \vspace{-7pt}
  \caption{\small{HV and SP performance on \texttt{Complete} datasets. (B: behavioral policy). The best scores are emphasized in bold. Please refer to \cref{app:Full Results} for the full results of the \texttt{Complete} datasets at the expert and amateur levels.}}
  \label{tab:complete_results_partial}
  \centering
  \resizebox{0.95\textwidth}{!}{
  \begin{tabular}{p{0.02\textwidth}p{0.1\textwidth}p{0.11\textwidth}||p{0.05\textwidth}|p{0.1\textwidth}p{0.1\textwidth}p{0.1\textwidth}p{0.1\textwidth}|p{0.1\textwidth}}
    \toprule
    ~ & \textbf{Env} & \textbf{Metrics} & \textbf{B} & \textbf{MODT(P)} & \textbf{MORvS(P)} & \textbf{BC(P)} & \textbf{CQL(P)} & \textbf{MODULI} \\
    \midrule
    \cmidrule[\heavyrulewidth]{1-9}
    \multirow{15}*{\rotatebox{90}{Expert}}  & \multirow{2}*{Ant}         & HV ($\times 10^{6}$) $\uparrow$ & 6.32 & 6.21±.01 & 6.36±.02 & 4.88±.17 & 5.76±.10 & \textbf{6.39±.02} \\
    ~                                       & ~                          & SP ($\times 10^{4}$) $\downarrow$ & - & 8.26±2.22 & 0.87±.19 & 46.20±16.40 & 0.58±.10 & \textbf{0.79±.12} \\
    \cmidrule{2-9}
    ~                                       & \multirow{2}*{HalfCheetah} & HV ($\times 10^{6}$) $\uparrow$ & 5.79 & 5.73±.00 & 5.78±.00 & 5.54±.05 & 5.63±.04 & \textbf{5.79±.00} \\
    ~                                       & ~                          & SP ($\times 10^{4}$) $\downarrow$ & - & 1.24±.23 & 0.67±.05 & 1.78±.39 & 0.10±.00 & \textbf{0.07±.00} \\
    \cmidrule{2-9}
    ~                                       & \multirow{2}*{Hopper}      & HV ($\times 10^{7}$) $\uparrow$ & 2.09 & 2.00±.02 & 2.02±.02 & 1.23±.10 & 0.33±.39 & \textbf{2.09±.01} \\
    ~                                       & ~                          & SP ($\times 10^{5}$) $\downarrow$ & - & 16.30±10.60 & 3.03±.36 & 52.50±4.88 & 2.84±2.46 & \textbf{0.09±.01} \\
    \cmidrule{2-9}
    ~                                       & \multirow{2}*{Swimmer}     & HV ($\times 10^{4}$) $\uparrow$ & 3.25 & 3.15±.02 & \textbf{3.24±.00} & 3.21±.00 & 3.22±.08 & \textbf{3.24±.00} \\
    ~                                       & ~                          & SP ($\times 10^{0}$) $\downarrow$ & - & 15.00±7.49 & \textbf{4.39±.07} & 4.50±.39 & 13.60±5.31 & 4.43±.38 \\
    \cmidrule{2-9}
    ~                                       & \multirow{2}*{Walker2d}    & HV ($\times 10^{6}$) $\uparrow$ & 5.21 & 4.89±.05 & 5.14±.01 & 3.74±.11 & 3.21±.32 & \textbf{5.20±.00} \\
    ~                                       & ~                          & SP ($\times 10^{4}$) $\downarrow$ & - & 0.99±.44 & 3.22±.73 & 75.60±52.30 & 6.23±10.70 & \textbf{0.11±.01} \\
    \cmidrule{2-9}
    ~                                       & \multirow{2}*{Hopper-3obj} & HV ($\times 10^{10}$) $\uparrow$ & 3.73 & 3.38±.05 & 3.42±.10 & 2.29±.07 & 0.78±.24 & \textbf{3.57±.02} \\
    ~                                       & ~                          & SP ($\times 10^{5}$) $\downarrow$ & - & 1.40±.44 & 2.72±1.93 & 0.72±.09 & 2.60±3.14 & \textbf{0.07±.00} \\

    \bottomrule
  \end{tabular}}
  \vspace{-5pt}
\end{table*}




% 完整版本表格 备份用 附录要用
% \begin{table*}[htb]
%   \small
%   \caption{Hv and Sp performance on \texttt{Complete} datasets. (B: behavioral policy). We report the mean per and standard error over 3 random seeds. The best scores are emphasized in bold.}
%   \label{tab:complete_results}
%   \centering
%   \begin{tabular}{p{0.02\textwidth}p{0.1\textwidth}p{0.11\textwidth}||p{0.05\textwidth}|p{0.1\textwidth}p{0.1\textwidth}p{0.1\textwidth}p{0.1\textwidth}|p{0.1\textwidth}}
%     \toprule
%     ~ & \textbf{Env} & \textbf{Metrics} & \textbf{B} & \textbf{MODT(P)} & \textbf{MORvS(P)} & \textbf{BC(P)} & \textbf{CQL(P)} & \textbf{MODULI} \\
%     \midrule
%     \multirow{15}*{\rotatebox{90}{Amateur}} & \multirow{2}*{Ant}         & HV ($\times 10^{6}$) $\uparrow$ & 5.61 & 5.92±.04 & 6.07±.02 & 4.37±.06 & 5.62±.23 & \textbf{6.08±.03} \\
%     ~                                       & ~                          & SP ($\times 10^{4}$) $\downarrow$ & - & 8.72±.77 & 5.24±.52 & 25.90±16.40 & 1.06±.28 & \textbf{0.53±.05} \\
%     \cmidrule{2-9}
%     ~                                       & \multirow{2}*{HalfCheetah} & HV ($\times 10^{6}$) $\uparrow$ & 5.68 & 5.69±.01 & \textbf{5.77±.00} & 5.46±.02 & 5.54±.02 & 5.76±.00 \\
%     ~                                       & ~                          & SP ($\times 10^{4}$) $\downarrow$ & - & 1.16±.42 & 0.57±.09 & 2.22±.91 & 0.45±.27 & \textbf{0.07±.02} \\
%     \cmidrule{2-9}
%     ~                                       & \multirow{2}*{Hopper}      & HV ($\times 10^{7}$) $\uparrow$ & 1.97 & 1.81±.05 & 1.76±.03 & 1.35±.03 & 1.64±.01 & \textbf{2.01±.01} \\
%     ~                                       & ~                          & SP ($\times 10^{5}$) $\downarrow$ & - & 1.61±.29 & 3.50±1.54 & 2.42±1.08 & 3.30±5.25 & \textbf{0.10±.01} \\
%     \cmidrule{2-9}
%     ~                                       & \multirow{2}*{Swimmer}     & HV ($\times 10^{4}$) $\uparrow$ & 2.11 & 1.67±.22 & 2.79±.03 & 2.82±.04 & 1.69±.93 & \textbf{3.20±.00} \\
%     ~                                       & ~                          & SP ($\times 10^{0}$) $\downarrow$ & - & 2.87±1.32 & \textbf{1.03±.20} & 5.05±1.82 & 8.87±6.24 & 9.50±.59 \\
%     \cmidrule{2-9}
%     ~                                       & \multirow{2}*{Walker2d}    & HV ($\times 10^{6}$) $\uparrow$ & 4.99 & 3.10±.34 & 4.98±.01 & 3.42±.42 & 1.78±.33 & \textbf{5.06±.00} \\
%     ~                                       & ~                          & SP ($\times 10^{4}$) $\downarrow$ & - & 164.20±13.50 & 1.94±.06 & 53.10±34.60 & 7.33±5.89 & \textbf{0.25±.03} \\
%     \cmidrule{2-9}
%     ~                                       & \multirow{2}*{Hopper-3obj} & HV ($\times 10^{10}$) $\uparrow$ & 3.09 & 1.04±.16 & 2.77±.24 & 2.42±.18 & 0.59±.42 & \textbf{3.33±.06} \\
%     ~                                       & ~                          & SP ($\times 10^{5}$) $\downarrow$ & - & 10.23±2.78 & 1.03±.11 & 0.87±.29 & 2.00±1.72 & \textbf{0.10±.00} \\
%     \cmidrule[\heavyrulewidth]{1-9}
%     \multirow{15}*{\rotatebox{90}{Expert}}  & \multirow{2}*{Ant}         & HV ($\times 10^{6}$) $\uparrow$ & 6.32 & 6.21±.01 & 6.36±.02 & 4.88±.17 & 5.76±.10 & \textbf{6.39±.02} \\
%     ~                                       & ~                          & SP ($\times 10^{4}$) $\downarrow$ & - & 8.26±2.22 & 0.87±.19 & 46.20±16.40 & 0.58±.10 & \textbf{0.79±.12} \\
%     \cmidrule{2-9}
%     ~                                       & \multirow{2}*{HalfCheetah} & HV ($\times 10^{6}$) $\uparrow$ & 5.79 & 5.73±.00 & 5.78±.00 & 5.54±.05 & 5.63±.04 & \textbf{5.79±.00} \\
%     ~                                       & ~                          & SP ($\times 10^{4}$) $\downarrow$ & - & 1.24±.23 & 0.67±.05 & 1.78±.39 & 0.10±.00 & \textbf{0.07±.00} \\
%     \cmidrule{2-9}
%     ~                                       & \multirow{2}*{Hopper}      & HV ($\times 10^{7}$) $\uparrow$ & 2.09 & 2.00±.02 & 2.02±.02 & 1.23±.10 & 0.33±.39 & \textbf{2.09±.01} \\
%     ~                                       & ~                          & SP ($\times 10^{5}$) $\downarrow$ & - & 16.30±10.60 & 3.03±.36 & 52.50±4.88 & 2.84±2.46 & \textbf{0.09±.01} \\
%     \cmidrule{2-9}
%     ~                                       & \multirow{2}*{Swimmer}     & HV ($\times 10^{4}$) $\uparrow$ & 3.25 & 3.15±.02 & \textbf{3.24±.00} & 3.21±.00 & 3.22±.08 & \textbf{3.24±.00} \\
%     ~                                       & ~                          & SP ($\times 10^{0}$) $\downarrow$ & - & 15.00±7.49 & \textbf{4.39±.07} & 4.50±.39 & 13.60±5.31 & 4.43±.38 \\
%     \cmidrule{2-9}
%     ~                                       & \multirow{2}*{Walker2d}    & HV ($\times 10^{6}$) $\uparrow$ & 5.21 & 4.89±.05 & 5.14±.01 & 3.74±.11 & 3.21±.32 & \textbf{5.20±.00} \\
%     ~                                       & ~                          & SP ($\times 10^{4}$) $\downarrow$ & - & 0.99±.44 & 3.22±.73 & 75.60±52.30 & 6.23±10.70 & \textbf{0.11±.01} \\
%     \cmidrule{2-9}
%     ~                                       & \multirow{2}*{Hopper-3obj} & HV ($\times 10^{10}$) $\uparrow$ & 3.73 & 3.38±.05 & 3.42±.10 & 2.29±.07 & 0.78±.24 & \textbf{3.57±.02} \\
%     ~                                       & ~                          & SP ($\times 10^{5}$) $\downarrow$ & - & 1.40±.44 & 2.72±1.93 & 0.72±.09 & 2.60±3.14 & \textbf{0.07±.00} \\

%     \bottomrule
%   \end{tabular}
% \end{table*}



==> tables/main_results_2.tex <==
\begin{table*}[htb]
  \caption{Shattered}
  \label{sample-table}
  \centering
  \begin{tabular}{p{0.03\textwidth}p{0.1\textwidth}p{0.11\textwidth}||p{0.1\textwidth}p{0.1\textwidth}p{0.1\textwidth}|p{0.1\textwidth}p{0.1\textwidth}}
    \toprule
    ~ & \textbf{Env} & metrics & \textbf{MODT(P)} & \textbf{MORvS(P)} & \textbf{BC(P)} & \textbf{MODULI} & \textbf{MODULI w slider} \\
    \midrule
    \multirow{20}*{\rotatebox{90}{Amateur}} & \multirow{3}*{Ant}         & HV ($\times 10^{6}$) & 5.74±.04 & \textbf{6.09±.01} & 4.20±.05 & 6.08±.01 & 6.06±.02 \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & 2.05±.02 & \textbf{2.11±.00} & 1.86±.01 & 2.08±.01 & 2.08±.01 \\
    ~                                       & ~                          & SP ($\times 10^{4}$) & 2.47±.61 & 0.79±.14 & 2.29±1.38 & 0.54±.04 & 0.60±.08 \\
    \cmidrule{2-8}
    ~                                       & \multirow{3}*{HalfCheetah} & HV ($\times 10^{6}$) & 5.61±.01 & 5.74±.00 & 5.54±.00 & \textbf{5.75±.00} & 5.73±.00 \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & \textbf{2.23±.00} & 2.11±.00 & 2.09±.00 & 2.07±.00 & 2.07±.01 \\
    ~                                       & ~                          & SP ($\times 10^{4}$) & 0.11±.01 & 0.09±.01 & 0.09±.01 & 0.13±.02 & 0.19±.02 \\
    \cmidrule{2-8}
    ~                                       & \multirow{3}*{Hopper}      & HV ($\times 10^{7}$) & 1.46±.00 & 1.69±.01 & 1.63±.00 & 2.00±.00 & \textbf{2.01±.00} \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & 3.90±.02 & 3.85±.02 & 3.70±.01 & 3.96±.00 & \textbf{4.00±.04} \\
    ~                                       & ~                          & SP ($\times 10^{5}$) & 0.54±.58 & 0.08±.01 & 0.11±.05 & 0.17±.02 & 0.19±.01 \\
    \cmidrule{2-8}
    ~                                       & \multirow{3}*{Swimmer}     & HV ($\times 10^{4}$) & 0.75±.00 & 2.81±.00 & 2.81±.00 & \textbf{3.18±.01} & \textbf{3.18±.00} \\
    ~                                       & ~                          & WR ($\times 10^{2}$) & 1.38±.00 & 1.43±.00 & 1.48±.00 & 1.62±.02 & \textbf{1.65±.02} \\
    ~                                       & ~                          & SP ($\times 10^{0}$) & 6.75±.23 & 1.26±.06 & 1.89±.05 & 8.85±.77 & 15.71±.61 \\
    \cmidrule{2-8}
    ~                                       & \multirow{3}*{Walker2d}    & HV ($\times 10^{6}$) & 3.86±.07 & 4.99±.00 & 3.42±.02 & \textbf{5.03±.01} & \textbf{5.03±.00} \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & 1.87±.01 & \textbf{1.98±.01} & 1.80±.01 & 1.93±.00 & 1.94±.00 \\
    ~                                       & ~                          & SP ($\times 10^{4}$) & 11.13±3.58 & 0.20±.03 & 4.56±.08 & 0.29±.01 & 0.33±.02 \\
    \cmidrule{2-8}
    ~                                       & \multirow{3}*{Hopper-3obj} & HV ($\times 10^{10}$) & 1.48±.02 & 2.84±.04 & 1.34±.02 & 2.99±.06 & \textbf{3.05±.10} \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & \textbf{2.55±.01} & 2.33±.02 & 1.82±.01 & 2.16±.01 & 2.20±.03 \\
    ~                                       & ~                          & SP ($\times 10^{5}$) & 0.56±.08 & 0.11±.01 & 0.59±.08 & 0.11±.01 & 0.10±.01 \\
    \cmidrule[\heavyrulewidth]{1-8}
    \multirow{27}*{\rotatebox{90}{Expert}}  & \multirow{3}*{Ant}         & HV ($\times 10^{6}$) & 5.88±.02 & 6.38±.01 & 4.76±.05 & 6.39±.02 & \textbf{6.40±.01} \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & 2.13±.02 & \textbf{2.15±.01} & 1.94±.02 & \textbf{2.15±.01} & \textbf{2.15±.01} \\
    ~                                       & ~                          & SP ($\times 10^{4}$) & 2.22±.50 & 0.75±.13 & 5.16±1.18 & 0.82±.25 & 0.71±.20 \\
    \cmidrule{2-8}
    ~                                       & \multirow{3}*{HalfCheetah} & HV ($\times 10^{6}$) & 5.69±.00 & 5.73±.00 & 5.66±.00 & \textbf{5.78±.00} & 5.77±.00 \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & \textbf{2.16±.00} & 2.13±.00 & 2.07±.01 & 2.09±.00 & 2.11±.00 \\
    ~                                       & ~                          & SP ($\times 10^{4}$) & 0.18±.01 & 0.15±.02 & 0.34±.03 & 0.10±.01 & 0.13±.01 \\
    \cmidrule{2-8}
    ~                                       & \multirow{3}*{Hopper}      & HV ($\times 10^{7}$) & 1.95±.03 & \textbf{2.07±.01} & 1.49±.01 & \textbf{2.07±.00} & \textbf{2.07±.00} \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & 4.02±.02 & \textbf{4.15±.03} & 3.66±.07 & 4.06±.01 & 4.05±.01 \\
    ~                                       & ~                          & SP ($\times 10^{5}$) & 0.85±.27 & 0.20±.06 & 2.58±1.01 & 0.11±.00 & 0.11±.02 \\
    \cmidrule{2-8}
    ~                                       & \multirow{3}*{Swimmer}     & HV ($\times 10^{4}$) & 3.20±.00 & \textbf{3.24±.00} & 3.19±.00 & \textbf{3.24±.00} & \textbf{3.24±.00} \\
    ~                                       & ~                          & WR ($\times 10^{2}$) & 1.56±.01 & \textbf{1.70±.01} & \textbf{1.70±.01} & 1.63±.01 & 1.64±.01 \\
    ~                                       & ~                          & SP ($\times 10^{0}$) & 15.50±.33 & 7.36±.81 & 9.05±.30 & 6.04±.48 & 9.03±1.08 \\
    \cmidrule{2-8}
    ~                                       & \multirow{3}*{Walker2d}    & HV ($\times 10^{6}$) & 5.01±.01 & 5.14±.01 & 3.47±.12 & \textbf{5.20±.00} & \textbf{5.20±.00} \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & \textbf{2.04±.00} & 1.98±.01 & 1.45±.04 & 1.96±.00 & 1.97±.00 \\
    ~                                       & ~                          & SP ($\times 10^{4}$) & 0.49±.03 & 0.27±.04 & 16.61±13.78 & 0.12±.00 & 0.14±.01 \\
    \cmidrule{2-8}
    ~                                       & \multirow{3}*{Hopper-3obj} & HV ($\times 10^{10}$) & 2.83±.06 & 3.28±.07 & 1.95±.16 & 3.36±.03 & \textbf{3.39±.04} \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & 2.16±.02 & \textbf{2.46±.00} & 1.96±.05 & 2.29±.01 & 2.27±.04 \\
    ~                                       & ~                          & SP ($\times 10^{5}$) & 0.09±.01 & 0.06±.00 & 0.17±.06 & 0.11±.01 & 0.12±.01 \\

    \bottomrule
  \end{tabular}
\end{table*}

% \begin{table*}[htb]
%   \caption{Shattered-ood}
%   \label{sample-table}
%   \centering
%   \begin{tabular}{p{0.03\textwidth}p{0.1\textwidth}p{0.11\textwidth}||p{0.1\textwidth}p{0.1\textwidth}p{0.1\textwidth}|p{0.1\textwidth}p{0.1\textwidth}}
%     \toprule
%     ~ & \textbf{Env} & metrics & \textbf{MODT(P)} & \textbf{MORvS(P)} & \textbf{BC(P)} & \textbf{MODULI} & \textbf{MODULI w slider} \\
%     \midrule
%     \multirow{27}*{\rotatebox{90}{Amateur}} & \multirow{4}*{Ant}         & HV ($\times 10^{6}$) & 5.74±.04 & \textbf{6.09±.01} & 4.20±.05 & 6.08±.01 & 6.06±.02 \\
%     ~                                       & ~                          & SP ($\times 10^{4}$) & 2.47±.61 & 0.79±.14 & 2.29±1.38 & \textbf{0.54±.04} & 0.60±.08 \\
%     ~                                       & ~                          & MV ($\times 10^{-1}$) & 0.59±.03 & 0.22±.02 & 0.61±.01 & \textbf{0.16±.00} & 0.17±.01 \\
%     ~                                       & ~                          & WR ($\times 10^{3}$) & 1.85±.01 & 1.97±.02 & 1.32±.05 & \textbf{2.01±.00} & 2.00±.01 \\
%     \cmidrule{2-8}
%     ~                                       & \multirow{4}*{HalfCheetah} & HV ($\times 10^{6}$) & 5.61±.01 & 5.74±.00 & 5.54±.00 & \textbf{5.75±.00} & 5.73±.00 \\
%     ~                                       & ~                          & SP ($\times 10^{4}$) & 0.11±.01 & \textbf{0.09±.01} & \textbf{0.09±.01} & 0.13±.02 & 0.19±.02 \\
%     ~                                       & ~                          & MV ($\times 10^{-1}$) & 2.35±.02 & 0.23±.00 & 0.47±.02 & 0.35±.03 & \textbf{0.16±.00} \\
%     ~                                       & ~                          & WR ($\times 10^{3}$) & \textbf{2.08±.00} & 2.06±.00 & 2.03±.00 & 2.04±.00 & 2.05±.00 \\
%     \cmidrule{2-8}
%     ~                                       & \multirow{4}*{Hopper}      & HV ($\times 10^{7}$) & 1.46±.00 & 1.69±.01 & 1.63±.00 & 2.00±.00 & \textbf{2.01±.00} \\
%     ~                                       & ~                          & SP ($\times 10^{5}$) & 0.54±.58 & \textbf{0.08±.01} & 0.11±.05 & 0.17±.02 & 0.19±.01 \\
%     ~                                       & ~                          & MV ($\times 10^{-1}$) & 1.36±.03 & 0.31±.01 & \textbf{0.22±.02} & 0.26±.01 & 0.25±.01 \\
%     ~                                       & ~                          & WR ($\times 10^{3}$) & 2.28±.01 & 2.82±.02 & 3.35±.04 & 3.77±.04 & \textbf{3.80±.06} \\
%     \cmidrule{2-8}
%     ~                                       & \multirow{4}*{Swimmer}     & HV ($\times 10^{4}$) & 0.75±.00 & 2.81±.00 & 2.81±.00 & \textbf{3.18±.01} & \textbf{3.18±.00} \\
%     ~                                       & ~                          & SP ($\times 10^{0}$) & 6.75±.23 & \textbf{1.26±.06} & 1.89±.05 & 8.85±.77 & 15.71±.61 \\
%     ~                                       & ~                          & MV ($\times 10^{-1}$) & \textbf{0.45±.02} & 1.50±.00 & 1.72±.01 & 0.53±.01 & 0.61±.03 \\
%     ~                                       & ~                          & WR ($\times 10^{2}$) & 0.91±.00 & 1.33±.00 & 1.34±.00 & \textbf{1.45±.00} & 1.44±.00 \\
%     \cmidrule{2-8}
%     ~                                       & \multirow{4}*{Walker2d}    & HV ($\times 10^{6}$) & 3.86±.07 & 4.99±.00 & 3.42±.02 & \textbf{5.03±.01} & \textbf{5.03±.00} \\
%     ~                                       & ~                          & SP ($\times 10^{4}$) & 11.13±3.58 & \textbf{0.20±.03} & 4.56±.08 & 0.29±.01 & 0.33±.02 \\
%     ~                                       & ~                          & MV ($\times 10^{-1}$) & 0.97±.26 & \textbf{0.18±.01} & 2.25±.05 & 0.19±.03 & 0.21±.01 \\
%     ~                                       & ~                          & WR ($\times 10^{3}$) & 0.89±.02 & \textbf{1.78±.00} & 1.18±.01 & 1.71±.01 & 1.71±.02 \\
%     \cmidrule{2-8}
%     ~                                       & \multirow{4}*{Hopper-3obj} & HV ($\times 10^{10}$) & 1.48±.02 & 2.84±.04 & 1.34±.02 & 2.99±.06 & \textbf{3.05±.10} \\
%     ~                                       & ~                          & SP ($\times 10^{5}$) & 0.56±.08 & 0.11±.01 & 0.59±.08 & 0.11±.01 & \textbf{0.10±.01} \\
%     ~                                       & ~                          & MV ($\times 10^{-1}$) & 2.60±.12 & 1.28±.06 & 2.07±.02 & \textbf{0.84±.04} & 1.03±.02 \\
%     ~                                       & ~                          & WR ($\times 10^{3}$) & 0.64±.00 & \textbf{1.88±.01} & 0.67±.00 & 1.67±.01 & 1.65±.01 \\
%     \cmidrule[\heavyrulewidth]{1-8}
%     \multirow{27}*{\rotatebox{90}{Expert}}  & \multirow{4}*{Ant}         & HV ($\times 10^{6}$) & 5.88±.02 & 6.38±.01 & 4.76±.05 & 6.39±.02 & \textbf{6.40±.01} \\
%     ~                                       & ~                          & SP ($\times 10^{4}$) & 2.22±.50 & 0.75±.13 & 5.16±1.18 & 0.82±.25 & \textbf{0.71±.20} \\
%     ~                                       & ~                          & MV ($\times 10^{-1}$) & 1.04±.07 & 0.16±.01 & 0.95±.08 & \textbf{0.15±.01} & 0.20±.04 \\
%     ~                                       & ~                          & WR ($\times 10^{3}$) & 1.68±.02 & 2.03±.00 & 1.81±.01 & \textbf{2.05±.00} & 2.04±.00 \\
%     \cmidrule{2-8}
%     ~                                       & \multirow{4}*{HalfCheetah} & HV ($\times 10^{6}$) & 5.69±.00 & 5.73±.00 & 5.66±.00 & \textbf{5.78±.00} & 5.77±.00 \\
%     ~                                       & ~                          & SP ($\times 10^{4}$) & 0.18±.01 & 0.15±.02 & 0.34±.03 & \textbf{0.10±.01} & 0.13±.01 \\
%     ~                                       & ~                          & MV ($\times 10^{-1}$) & 0.74±.02 & 0.43±.00 & 0.57±.04 & \textbf{0.17±.01} & 0.28±.02 \\
%     ~                                       & ~                          & WR ($\times 10^{3}$) & \textbf{2.08±.00} & 2.05±.00 & 2.02±.00 & 2.07±.00 & 2.07±.00 \\
%     \cmidrule{2-8}
%     ~                                       & \multirow{4}*{Hopper}      & HV ($\times 10^{7}$) & 1.95±.03 & \textbf{2.07±.01} & 1.49±.01 & \textbf{2.07±.00} & \textbf{2.07±.00} \\
%     ~                                       & ~                          & SP ($\times 10^{5}$) & 0.85±.27 & 0.20±.06 & 2.58±1.01 & \textbf{0.11±.00} & \textbf{0.11±.02} \\
%     ~                                       & ~                          & MV ($\times 10^{-1}$) & 0.84±.25 & 0.16±.02 & 1.51±.16 & \textbf{0.09±.01} & \textbf{0.09±.01} \\
%     ~                                       & ~                          & WR ($\times 10^{3}$) & 3.32±.01 & 3.38±.03 & 1.35±.08 & \textbf{3.97±.03} & \textbf{3.97±.07} \\
%     \cmidrule{2-8}
%     ~                                       & \multirow{4}*{Swimmer}     & HV ($\times 10^{4}$) & 3.20±.00 & \textbf{3.24±.00} & 3.19±.00 & \textbf{3.24±.00} & \textbf{3.24±.00} \\
%     ~                                       & ~                          & SP ($\times 10^{0}$) & 15.50±.33 & 7.36±.81 & 9.05±.30 & \textbf{6.04±.48} & 9.03±1.08 \\
%     ~                                       & ~                          & MV ($\times 10^{-1}$) & 0.61±.01 & 0.18±.01 & 0.63±.03 & \textbf{0.12±.02} & 0.16±.01 \\
%     ~                                       & ~                          & WR ($\times 10^{2}$) & 1.31±.00 & 1.41±.00 & \textbf{1.45±.00} & \textbf{1.45±.00} & \textbf{1.45±.00} \\
%     \cmidrule{2-8}
%     ~                                       & \multirow{4}*{Walker2d}    & HV ($\times 10^{6}$) & 5.01±.01 & 5.14±.01 & 3.47±.12 & \textbf{5.20±.00} & \textbf{5.20±.00} \\
%     ~                                       & ~                          & SP ($\times 10^{4}$) & 0.49±.03 & 0.27±.04 & 16.61±13.78 & \textbf{0.12±.00} & 0.14±.01 \\
%     ~                                       & ~                          & MV ($\times 10^{-1}$) & 0.53±.01 & 0.16±.01 & 4.52±.57 & \textbf{0.14±.01} & 0.16±.01 \\
%     ~                                       & ~                          & WR ($\times 10^{3}$) & 1.39±.02 & 1.50±.01 & 0.72±.01 & 1.88±.01 & \textbf{1.90±.00} \\
%     \cmidrule{2-8}
%     ~                                       & \multirow{4}*{Hopper-3obj} & HV ($\times 10^{10}$) & 2.83±.06 & 3.28±.07 & 1.95±.16 & 3.36±.03 & \textbf{3.39±.04} \\
%     ~                                       & ~                          & SP ($\times 10^{5}$) & 0.09±.01 & \textbf{0.06±.00} & 0.17±.06 & 0.11±.01 & 0.12±.01 \\
%     ~                                       & ~                          & MV ($\times 10^{-1}$) & 1.64±.05 & 1.23±.01 & 2.41±.11 & \textbf{0.93±.03} & 0.99±.08 \\
%     ~                                       & ~                          & WR ($\times 10^{3}$) & \textbf{1.84±.01} & \textbf{1.84±.02} & 0.68±.01 & 1.71±.02 & 1.81±.04 \\

%     \bottomrule
%   \end{tabular}
% \end{table*}

\begin{table*}[htb]
  \caption{Narrow}
  \label{sample-table}
  \centering
  \begin{tabular}{p{0.03\textwidth}p{0.1\textwidth}p{0.11\textwidth}||p{0.1\textwidth}p{0.1\textwidth}p{0.1\textwidth}|p{0.1\textwidth}p{0.1\textwidth}}
    \toprule
    ~ & \textbf{Env} & metrics & \textbf{MODT(P)} & \textbf{MORvS(P)} & \textbf{BC(P)} & \textbf{MODULI} & \textbf{MODULI w slider} \\
    \midrule
    \multirow{20}*{\rotatebox{90}{Amateur}} & \multirow{3}*{Ant}         & HV ($\times 10^{6}$) & 5.17±.03 & 5.80±.03 & 4.19±.10 & 5.85±.03 & \textbf{5.86±.02} \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & \textbf{2.07±.02} & \textbf{2.07±.01} & 1.76±.06 & 2.05±.00 & 2.06±.00 \\
    ~                                       & ~                          & SP ($\times 10^{4}$) & 0.43±.10 & 0.51±.08 & 4.42±1.44 & 0.62±.11 & 0.61±.09 \\
    \cmidrule{2-8}
    ~                                       & \multirow{3}*{HalfCheetah} & HV ($\times 10^{6}$) & 4.29±.00 & 5.55±.00 & 5.08±.01 & 5.72±.00 & \textbf{5.73±.00} \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & 2.15±.04 & 2.10±.00 & 2.12±.00 & 2.10±.00 & \textbf{2.17±.01} \\
    ~                                       & ~                          & SP ($\times 10^{4}$) & 1.02±.44 & 0.02±.00 & 0.02±.00 & 0.06±.00 & 0.05±.00 \\
    \cmidrule{2-8}
    ~                                       & \multirow{3}*{Hopper}      & HV ($\times 10^{7}$) & 1.73±.01 & 1.69±.01 & 0.94±.34 & 1.99±.01 & \textbf{2.01±.01} \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & 3.84±.01 & 3.90±.02 & 3.01±.58 & 3.96±.06 & \textbf{3.99±.01} \\
    ~                                       & ~                          & SP ($\times 10^{5}$) & 0.27±.07 & 0.15±.03 & 5.81±8.21 & 0.37±.18 & 0.18±.02 \\
    \cmidrule{2-8}
    ~                                       & \multirow{3}*{Swimmer}     & HV ($\times 10^{4}$) & 0.66±.03 & 2.95±.00 & 2.80±.00 & 3.14±.00 & \textbf{3.16±.00} \\
    ~                                       & ~                          & WR ($\times 10^{2}$) & 1.37±.05 & 1.48±.00 & 1.39±.00 & 1.59±.01 & \textbf{1.63±.01} \\
    ~                                       & ~                          & SP ($\times 10^{0}$) & 14.25±3.73 & 1.91±.01 & 2.95±.08 & 11.56±1.28 & 10.54±1.45 \\
    \cmidrule{2-8}
    ~                                       & \multirow{3}*{Walker2d}    & HV ($\times 10^{6}$) & 3.42±.16 & 4.83±.00 & 2.83±.01 & 4.91±.01 & \textbf{4.93±.00} \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & 1.75±.01 & 1.92±.00 & 1.76±.00 & 1.92±.00 & \textbf{1.94±.00} \\
    ~                                       & ~                          & SP ($\times 10^{4}$) & 5.64±3.72 & 0.22±.01 & 0.01±.00 & 0.24±.01 & 0.25±.01 \\
    \cmidrule{2-8}
    ~                                       & \multirow{3}*{Hopper-3obj} & HV ($\times 10^{10}$) & 1.85±.04 & 2.27±.05 & 2.26±.02 & 2.85±.06 & \textbf{2.96±.08} \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & \textbf{2.52±.03} & 2.15±.01 & 2.03±.01 & 2.11±.01 & 2.12±.02 \\
    ~                                       & ~                          & SP ($\times 10^{5}$) & 3.12±1.21 & 0.07±.01 & 0.09±.00 & 0.13±.01 & 0.12±.02 \\
    \cmidrule[\heavyrulewidth]{1-8}
    \multirow{27}*{\rotatebox{90}{Expert}}  & \multirow{3}*{Ant}         & HV ($\times 10^{6}$) & 5.05±.08 & 6.06±.00 & 4.90±.02 & \textbf{6.35±.01} & 6.31±.02 \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & 2.06±.02 & 2.11±.01 & 1.94±.02 & 2.19±.02 & \textbf{2.21±.03} \\
    ~                                       & ~                          & SP ($\times 10^{4}$) & 0.88±.41 & 0.79±.11 & 1.56±.28 & 0.73±.07 & 0.68±.16 \\
    \cmidrule{2-8}
    ~                                       & \multirow{3}*{HalfCheetah} & HV ($\times 10^{6}$) & 5.04±.00 & 5.46±.01 & 4.88±.02 & \textbf{5.76±.00} & \textbf{5.76±.00} \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & \textbf{2.16±.00} & 2.07±.00 & 2.13±.00 & 2.13±.01 & 2.13±.00 \\
    ~                                       & ~                          & SP ($\times 10^{4}$) & 0.04±.00 & 0.05±.00 & 0.02±.00 & 0.04±.00 & 0.04±.00 \\
    \cmidrule{2-8}
    ~                                       & \multirow{3}*{Hopper}      & HV ($\times 10^{7}$) & 1.85±.02 & 1.98±.00 & 1.29±.01 & \textbf{2.03±.01} & 2.02±.00 \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & \textbf{4.22±.02} & 4.09±.03 & 3.39±.02 & 4.06±.03 & 3.99±.00 \\
    ~                                       & ~                          & SP ($\times 10^{5}$) & 0.34±.07 & 0.16±.02 & 0.59±.24 & 0.30±.12 & 0.25±.04 \\
    \cmidrule{2-8}
    ~                                       & \multirow{3}*{Swimmer}     & HV ($\times 10^{4}$) & 3.03±.00 & 3.10±.00 & 3.06±.00 & \textbf{3.21±.00} & \textbf{3.21±.00} \\
    ~                                       & ~                          & WR ($\times 10^{2}$) & 1.52±.01 & 1.51±.01 & 1.50±.01 & 1.55±.01 & \textbf{1.63±.01} \\
    ~                                       & ~                          & SP ($\times 10^{0}$) & 3.65±.22 & 4.38±.80 & 5.53±.20 & 3.24±.13 & 2.93±.10 \\
    \cmidrule{2-8}
    ~                                       & \multirow{3}*{Walker2d}    & HV ($\times 10^{6}$) & 4.75±.01 & 4.85±.01 & 1.88±.95 & \textbf{5.10±.01} & 5.07±.01 \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & 1.90±.01 & 1.94±.00 & 0.92±.26 & 1.96±.00 & \textbf{1.99±.00} \\
    ~                                       & ~                          & SP ($\times 10^{4}$) & 0.34±.09 & 0.19±.02 & 10.76±11.58 & 0.15±.04 & 0.13±.01 \\
    \cmidrule{2-8}
    ~                                       & \multirow{3}*{Hopper-3obj} & HV ($\times 10^{10}$) & 3.18±.05 & 3.32±.00 & 2.32±.10 & 3.33±.04 & \textbf{3.34±.05} \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & 2.30±.03 & \textbf{2.44±.02} & 2.01±.01 & 2.29±.03 & 2.23±.02 \\
    ~                                       & ~                          & SP ($\times 10^{5}$) & 0.11±.01 & 0.22±.02 & 0.14±.02 & 0.14±.02 & 0.12±.01 \\

    \bottomrule
  \end{tabular}
\end{table*}

% \begin{table*}[htb]
%   \caption{Narrow-ood}
%   \label{sample-table}
%   \centering
%   \begin{tabular}{p{0.03\textwidth}p{0.1\textwidth}p{0.11\textwidth}||p{0.1\textwidth}p{0.1\textwidth}p{0.1\textwidth}|p{0.1\textwidth}p{0.1\textwidth}}
%     \toprule
%     ~ & \textbf{Env} & metrics & \textbf{MODT(P)} & \textbf{MORvS(P)} & \textbf{BC(P)} & \textbf{MODULI} & \textbf{MODULI w slider} \\
%     \midrule
%     \multirow{27}*{\rotatebox{90}{Amateur}} & \multirow{4}*{Ant}         & HV ($\times 10^{6}$) & 5.17±.03 & 5.80±.03 & 4.19±.10 & 5.85±.03 & \textbf{5.86±.02} \\
%     ~                                       & ~                          & SP ($\times 10^{4}$) & \textbf{0.43±.10} & 0.51±.08 & 4.42±1.44 & 0.62±.11 & 0.61±.09 \\
%     ~                                       & ~                          & MV ($\times 10^{-1}$) & 2.43±.16 & 0.34±.08 & 1.22±.24 & 0.20±.02 & \textbf{0.19±.02} \\
%     ~                                       & ~                          & WR ($\times 10^{3}$) & 1.94±.01 & \textbf{2.03±.02} & 0.71±.03 & 1.87±.01 & 2.01±.01 \\
%     \cmidrule{2-8}
%     ~                                       & \multirow{4}*{HalfCheetah} & HV ($\times 10^{6}$) & 4.29±.00 & 5.55±.00 & 5.08±.01 & 5.72±.00 & \textbf{5.73±.00} \\
%     ~                                       & ~                          & SP ($\times 10^{4}$) & 1.02±.44 & \textbf{0.02±.00} & \textbf{0.02±.00} & 0.06±.00 & 0.05±.00 \\
%     ~                                       & ~                          & MV ($\times 10^{-1}$) & 2.54±.16 & 0.34±.03 & 0.40±.02 & \textbf{0.29±.00} & 0.75±.02 \\
%     ~                                       & ~                          & WR ($\times 10^{3}$) & 2.01±.00 & \textbf{2.17±.00} & 2.11±.00 & 1.89±.00 & 2.08±.01 \\
%     \cmidrule{2-8}
%     ~                                       & \multirow{4}*{Hopper}      & HV ($\times 10^{7}$) & 1.73±.01 & 1.69±.01 & 0.94±.34 & 1.99±.01 & \textbf{2.01±.01} \\
%     ~                                       & ~                          & SP ($\times 10^{5}$) & 0.27±.07 & \textbf{0.15±.03} & 5.81±8.21 & 0.37±.18 & 0.18±.02 \\
%     ~                                       & ~                          & MV ($\times 10^{-1}$) & 0.86±.06 & 0.43±.00 & 1.46±.94 & \textbf{0.28±.01} & 0.29±.02 \\
%     ~                                       & ~                          & WR ($\times 10^{3}$) & 3.10±.04 & 2.00±.06 & 0.25±.00 & 3.34±.09 & \textbf{3.66±.06} \\
%     \cmidrule{2-8}
%     ~                                       & \multirow{4}*{Swimmer}     & HV ($\times 10^{4}$) & 0.66±.03 & 2.95±.00 & 2.80±.00 & 3.14±.00 & \textbf{3.16±.00} \\
%     ~                                       & ~                          & SP ($\times 10^{0}$) & 14.25±3.73 & \textbf{1.91±.01} & 2.95±.08 & 11.56±1.28 & 10.54±1.45 \\
%     ~                                       & ~                          & MV ($\times 10^{-1}$) & 0.66±.20 & 1.33±.00 & 1.46±.00 & \textbf{0.39±.02} & 0.50±.02 \\
%     ~                                       & ~                          & WR ($\times 10^{2}$) & 0.95±.00 & 1.57±.00 & 1.56±.00 & \textbf{1.69±.00} & 1.68±.00 \\
%     \cmidrule{2-8}
%     ~                                       & \multirow{4}*{Walker2d}    & HV ($\times 10^{6}$) & 3.42±.16 & 4.83±.00 & 2.83±.01 & 4.91±.01 & \textbf{4.93±.00} \\
%     ~                                       & ~                          & SP ($\times 10^{4}$) & 5.64±3.72 & 0.22±.01 & \textbf{0.01±.00} & 0.24±.01 & 0.25±.01 \\
%     ~                                       & ~                          & MV ($\times 10^{-1}$) & 1.32±.14 & 0.21±.00 & 1.58±.05 & \textbf{0.16±.00} & 0.27±.01 \\
%     ~                                       & ~                          & WR ($\times 10^{3}$) & 0.49±.00 & 0.60±.00 & 0.54±.00 & 1.24±.01 & \textbf{1.39±.02} \\
%     \cmidrule{2-8}
%     ~                                       & \multirow{4}*{Hopper-3obj} & HV ($\times 10^{10}$) & 1.85±.04 & 2.27±.05 & 2.26±.02 & 2.85±.06 & \textbf{2.96±.08} \\
%     ~                                       & ~                          & SP ($\times 10^{5}$) & 3.12±1.21 & \textbf{0.07±.01} & 0.09±.00 & 0.13±.01 & 0.12±.02 \\
%     ~                                       & ~                          & MV ($\times 10^{-1}$) & 2.30±.16 & 1.19±.02 & 1.82±.02 & \textbf{0.98±.05} & 1.32±.02 \\
%     ~                                       & ~                          & WR ($\times 10^{3}$) & 1.12±.01 & \textbf{1.63±.01} & 1.41±.01 & 1.21±.02 & 1.51±.02 \\
%     \cmidrule[\heavyrulewidth]{1-8}
%     \multirow{27}*{\rotatebox{90}{Expert}}  & \multirow{4}*{Ant}         & HV ($\times 10^{6}$) & 5.05±.08 & 6.06±.00 & 4.90±.02 & \textbf{6.35±.01} & 6.31±.02 \\
%     ~                                       & ~                          & SP ($\times 10^{4}$) & 0.88±.41 & 0.79±.11 & 1.56±.28 & 0.73±.07 & \textbf{0.68±.16} \\
%     ~                                       & ~                          & MV ($\times 10^{-1}$) & 2.59±.38 & \textbf{0.24±.04} & 1.12±.12 & 0.72±.12 & 1.01±.17 \\
%     ~                                       & ~                          & WR ($\times 10^{3}$) & 1.92±.00 & 2.02±.02 & 1.83±.03 & \textbf{2.16±.00} & \textbf{2.16±.01} \\
%     \cmidrule{2-8}
%     ~                                       & \multirow{4}*{HalfCheetah} & HV ($\times 10^{6}$) & 5.04±.00 & 5.46±.01 & 4.88±.02 & \textbf{5.76±.00} & \textbf{5.76±.00} \\
%     ~                                       & ~                          & SP ($\times 10^{4}$) & 0.04±.00 & 0.05±.00 & \textbf{0.02±.00} & 0.04±.00 & 0.04±.00 \\
%     ~                                       & ~                          & MV ($\times 10^{-1}$) & 1.36±.05 & \textbf{0.25±.02} & 1.00±.01 & 0.73±.01 & 0.57±.01 \\
%     ~                                       & ~                          & WR ($\times 10^{3}$) & 2.13±.00 & 2.16±.00 & 2.10±.00 & 2.17±.00 & \textbf{2.18±.00} \\
%     \cmidrule{2-8}
%     ~                                       & \multirow{4}*{Hopper}      & HV ($\times 10^{7}$) & 1.85±.02 & 1.98±.00 & 1.29±.01 & \textbf{2.03±.01} & 2.02±.00 \\
%     ~                                       & ~                          & SP ($\times 10^{5}$) & 0.34±.07 & \textbf{0.16±.02} & 0.59±.24 & 0.30±.12 & 0.25±.04 \\
%     ~                                       & ~                          & MV ($\times 10^{-1}$) & 1.22±.09 & 0.18±.01 & 0.62±.06 & \textbf{0.08±.03} & 0.11±.01 \\
%     ~                                       & ~                          & WR ($\times 10^{3}$) & 1.05±.01 & 3.18±.04 & 1.32±.04 & 2.25±.04 & \textbf{3.61±.06} \\
%     \cmidrule{2-8}
%     ~                                       & \multirow{4}*{Swimmer}     & HV ($\times 10^{4}$) & 3.03±.00 & 3.10±.00 & 3.06±.00 & \textbf{3.21±.00} & \textbf{3.21±.00} \\
%     ~                                       & ~                          & SP ($\times 10^{0}$) & 3.65±.22 & 4.38±.80 & 5.53±.20 & 3.24±.13 & \textbf{2.93±.10} \\
%     ~                                       & ~                          & MV ($\times 10^{-1}$) & 0.66±.00 & 0.45±.02 & 0.26±.01 & \textbf{0.08±.00} & 0.24±.00 \\
%     ~                                       & ~                          & WR ($\times 10^{2}$) & 1.66±.00 & 1.58±.01 & 1.66±.00 & \textbf{1.71±.00} & \textbf{1.71±.00} \\
%     \cmidrule{2-8}
%     ~                                       & \multirow{4}*{Walker2d}    & HV ($\times 10^{6}$) & 4.75±.01 & 4.85±.01 & 1.88±.95 & \textbf{5.10±.01} & 5.07±.01 \\
%     ~                                       & ~                          & SP ($\times 10^{4}$) & 0.34±.09 & 0.19±.02 & 10.76±11.58 & 0.15±.04 & \textbf{0.13±.01} \\
%     ~                                       & ~                          & MV ($\times 10^{-1}$) & 0.95±.10 & 0.30±.02 & 8.20±.18 & \textbf{0.21±.02} & 0.47±.01 \\
%     ~                                       & ~                          & WR ($\times 10^{3}$) & 1.28±.01 & 0.89±.02 & 0.56±.00 & 1.75±.02 & \textbf{1.99±.00} \\
%     \cmidrule{2-8}
%     ~                                       & \multirow{4}*{Hopper-3obj} & HV ($\times 10^{10}$) & 3.18±.05 & 3.32±.00 & 2.32±.10 & 3.33±.04 & \textbf{3.34±.05} \\
%     ~                                       & ~                          & SP ($\times 10^{5}$) & \textbf{0.11±.01} & 0.22±.02 & 0.14±.02 & 0.14±.02 & 0.12±.01 \\
%     ~                                       & ~                          & MV ($\times 10^{-1}$) & 1.38±.01 & 1.22±.03 & 2.47±.08 & \textbf{0.75±.04} & 1.16±.05 \\
%     ~                                       & ~                          & WR ($\times 10^{3}$) & 1.44±.00 & \textbf{1.63±.00} & 1.47±.02 & 1.33±.02 & 1.50±.03 \\

%     \bottomrule
%   \end{tabular}
% \end{table*}

==> tables/results_no_dyna.tex <==
\begin{table*}[tb]
  \caption{HV and SP performance on full \texttt{Complete} datasets. (B: behavioral policy). The best scores are emphasized in bold.}
  \label{tab:complete_results}
  \centering
  \resizebox{0.95\textwidth}{!}{
  \begin{tabular}{p{0.02\textwidth}p{0.1\textwidth}p{0.12\textwidth}||p{0.05\textwidth}|p{0.1\textwidth}p{0.1\textwidth}p{0.1\textwidth}p{0.1\textwidth}|p{0.1\textwidth}p{0.1\textwidth}}
    \toprule
    ~ & \textbf{Env} & \textbf{Metrics} & \textbf{B} & \textbf{MODT(P)} & \textbf{MORvS(P)} & \textbf{BC(P)} & \textbf{CQL(P)} & \textbf{MODULI} & \textbf{w/o invdyn} \\
    \midrule
    \multirow{15}*{\rotatebox{90}{Amateur}} & \multirow{2}*{Ant}         & HV ($\times 10^{6}$) $\uparrow$ & 5.61 & 5.92±.04 & 6.07±.02 & 4.37±.06 & 5.62±.23 & \textbf{6.08±.03} & 6.08\\
    ~                                       & ~                          & SP ($\times 10^{4}$) $\downarrow$ & - & 8.72±.77 & 5.24±.52 & 25.90±16.40 & 1.06±.28 & \textbf{0.53±.05} & /\\
    \cmidrule{2-10}
    ~                                       & \multirow{2}*{HalfCheetah} & HV ($\times 10^{6}$) $\uparrow$ & 5.68 & 5.69±.01 & \textbf{5.77±.00} & 5.46±.02 & 5.54±.02 & 5.76±.00 & /\\
    ~                                       & ~                          & SP ($\times 10^{4}$) $\downarrow$ & - & 1.16±.42 & 0.57±.09 & 2.22±.91 & 0.45±.27 & \textbf{0.07±.02} & /\\
    \cmidrule{2-10}
    ~                                       & \multirow{2}*{Hopper}      & HV ($\times 10^{7}$) $\uparrow$ & 1.97 & 1.81±.05 & 1.76±.03 & 1.35±.03 & 1.64±.01 & \textbf{2.01±.01} & 1.88\\
    ~                                       & ~                          & SP ($\times 10^{5}$) $\downarrow$ & - & 1.61±.29 & 3.50±1.54 & 2.42±1.08 & 3.30±5.25 & \textbf{0.10±.01} & /\\
    \cmidrule{2-10}
    ~                                       & \multirow{2}*{Swimmer}     & HV ($\times 10^{4}$) $\uparrow$ & 2.11 & 1.67±.22 & 2.79±.03 & 2.82±.04 & 1.69±.93 & \textbf{3.20±.00} & 3.11\\
    ~                                       & ~                          & SP ($\times 10^{0}$) $\downarrow$ & - & 2.87±1.32 & \textbf{1.03±.20} & 5.05±1.82 & 8.87±6.24 & 9.50±.59 & /\\
    \cmidrule{2-10}
    ~                                       & \multirow{2}*{Walker2d}    & HV ($\times 10^{6}$) $\uparrow$ & 4.99 & 3.10±.34 & 4.98±.01 & 3.42±.42 & 1.78±.33 & \textbf{5.06±.00} & /\\
    ~                                       & ~                          & SP ($\times 10^{4}$) $\downarrow$ & - & 164.20±13.50 & 1.94±.06 & 53.10±34.60 & 7.33±5.89 & \textbf{0.25±.03} & /\\
    \cmidrule{2-10}
    ~                                       & \multirow{2}*{Hopper-3obj} & HV ($\times 10^{10}$) $\uparrow$ & 3.09 & 1.04±.16 & 2.77±.24 & 2.42±.18 & 0.59±.42 & \textbf{3.33±.06} & /\\
    ~                                       & ~                          & SP ($\times 10^{5}$) $\downarrow$ & - & 10.23±2.78 & 1.03±.11 & 0.87±.29 & 2.00±1.72 & \textbf{0.10±.00} & /\\
    \cmidrule[\heavyrulewidth]{1-10}
    \multirow{15}*{\rotatebox{90}{Expert}}  & \multirow{2}*{Ant}         & HV ($\times 10^{6}$) $\uparrow$ & 6.32 & 6.21±.01 & 6.36±.02 & 4.88±.17 & 5.76±.10 & \textbf{6.39±.02} & 6.28\\
    ~                                       & ~                          & SP ($\times 10^{4}$) $\downarrow$ & - & 8.26±2.22 & 0.87±.19 & 46.20±16.40 & 0.58±.10 & \textbf{0.79±.12} & /\\
    \cmidrule{2-10}
    ~                                       & \multirow{2}*{HalfCheetah} & HV ($\times 10^{6}$) $\uparrow$ & 5.79 & 5.73±.00 & 5.78±.00 & 5.54±.05 & 5.63±.04 & \textbf{5.79±.00} & /\\
    ~                                       & ~                          & SP ($\times 10^{4}$) $\downarrow$ & - & 1.24±.23 & 0.67±.05 & 1.78±.39 & 0.10±.00 & \textbf{0.07±.00} & /\\
    \cmidrule{2-10}
    ~                                       & \multirow{2}*{Hopper}      & HV ($\times 10^{7}$) $\uparrow$ & 2.09 & 2.00±.02 & 2.02±.02 & 1.23±.10 & 0.33±.39 & \textbf{2.09±.01} & 1.94\\
    ~                                       & ~                          & SP ($\times 10^{5}$) $\downarrow$ & - & 16.30±10.60 & 3.03±.36 & 52.50±4.88 & 2.84±2.46 & \textbf{0.09±.01} & /\\
    \cmidrule{2-10}
    ~                                       & \multirow{2}*{Swimmer}     & HV ($\times 10^{4}$) $\uparrow$ & 3.25 & 3.15±.02 & \textbf{3.24±.00} & 3.21±.00 & 3.22±.08 & \textbf{3.24±.00} & 3.23\\
    ~                                       & ~                          & SP ($\times 10^{0}$) $\downarrow$ & - & 15.00±7.49 & \textbf{4.39±.07} & 4.50±.39 & 13.60±5.31 & 4.43±.38 & /\\
    \cmidrule{2-10}
    ~                                       & \multirow{2}*{Walker2d}    & HV ($\times 10^{6}$) $\uparrow$ & 5.21 & 4.89±.05 & 5.14±.01 & 3.74±.11 & 3.21±.32 & \textbf{5.20±.00} \\
    ~                                       & ~                          & SP ($\times 10^{4}$) $\downarrow$ & - & 0.99±.44 & 3.22±.73 & 75.60±52.30 & 6.23±10.70 & \textbf{0.11±.01} & /\\
    \cmidrule{2-10}
    ~                                       & \multirow{2}*{Hopper-3obj} & HV ($\times 10^{10}$) $\uparrow$ & 3.73 & 3.38±.05 & 3.42±.10 & 2.29±.07 & 0.78±.24 & \textbf{3.57±.02} \\
    ~                                       & ~                          & SP ($\times 10^{5}$) $\downarrow$ & - & 1.40±.44 & 2.72±1.93 & 0.72±.09 & 2.60±3.14 & \textbf{0.07±.00} & /\\

    \bottomrule
  \end{tabular}}
\end{table*}

==> tables/shattered_full.tex <==
\begin{table*}[htb]
  \caption{Shattered}
  \label{sample-table}
  \centering
  \begin{tabular}{p{0.03\textwidth}p{0.1\textwidth}p{0.11\textwidth}||p{0.1\textwidth}p{0.1\textwidth}p{0.1\textwidth}|p{0.1\textwidth}p{0.1\textwidth}}
    \toprule
    ~ & \textbf{Env} & metrics & \textbf{MODT(P)} & \textbf{MORvS(P)} & \textbf{BC(P)} & \textbf{MODULI} & \textbf{MODULI w slider} \\
    \midrule
    \multirow{20}*{\rotatebox{90}{Amateur}} & \multirow{3}*{Ant}         & HV ($\times 10^{6}$) & 5.74±.04 & \textbf{6.09±.01} & 4.20±.05 & 6.08±.01 & 6.06±.02 \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & 2.05±.02 & \textbf{2.11±.00} & 1.86±.01 & 2.08±.01 & 2.08±.01 \\
    ~                                       & ~                          & SP ($\times 10^{4}$) & 2.47±.61 & 0.79±.14 & 2.29±1.38 & 0.54±.04 & 0.60±.08 \\
    \cmidrule{2-8}
    ~                                       & \multirow{3}*{HalfCheetah} & HV ($\times 10^{6}$) & 5.61±.01 & 5.74±.00 & 5.54±.00 & \textbf{5.75±.00} & 5.73±.00 \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & \textbf{2.23±.00} & 2.11±.00 & 2.09±.00 & 2.07±.00 & 2.07±.01 \\
    ~                                       & ~                          & SP ($\times 10^{4}$) & 0.11±.01 & 0.09±.01 & 0.09±.01 & 0.13±.02 & 0.19±.02 \\
    \cmidrule{2-8}
    ~                                       & \multirow{3}*{Hopper}      & HV ($\times 10^{7}$) & 1.46±.00 & 1.69±.01 & 1.63±.00 & 2.00±.00 & \textbf{2.01±.00} \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & 3.90±.02 & 3.85±.02 & 3.70±.01 & 3.96±.00 & \textbf{4.00±.04} \\
    ~                                       & ~                          & SP ($\times 10^{5}$) & 0.54±.58 & 0.08±.01 & 0.11±.05 & 0.17±.02 & 0.19±.01 \\
    \cmidrule{2-8}
    ~                                       & \multirow{3}*{Swimmer}     & HV ($\times 10^{4}$) & 0.75±.00 & 2.81±.00 & 2.81±.00 & \textbf{3.18±.01} & \textbf{3.18±.00} \\
    ~                                       & ~                          & WR ($\times 10^{2}$) & 1.38±.00 & 1.43±.00 & 1.48±.00 & 1.62±.02 & \textbf{1.65±.02} \\
    ~                                       & ~                          & SP ($\times 10^{0}$) & 6.75±.23 & 1.26±.06 & 1.89±.05 & 8.85±.77 & 15.71±.61 \\
    \cmidrule{2-8}
    ~                                       & \multirow{3}*{Walker2d}    & HV ($\times 10^{6}$) & 3.86±.07 & 4.99±.00 & 3.42±.02 & \textbf{5.03±.01} & \textbf{5.03±.00} \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & 1.87±.01 & \textbf{1.98±.01} & 1.80±.01 & 1.93±.00 & 1.94±.00 \\
    ~                                       & ~                          & SP ($\times 10^{4}$) & 11.13±3.58 & 0.20±.03 & 4.56±.08 & 0.29±.01 & 0.33±.02 \\
    \cmidrule{2-8}
    ~                                       & \multirow{3}*{Hopper-3obj} & HV ($\times 10^{10}$) & 1.48±.02 & 2.84±.04 & 1.34±.02 & 2.99±.06 & \textbf{3.05±.10} \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & \textbf{2.55±.01} & 2.33±.02 & 1.82±.01 & 2.16±.01 & 2.20±.03 \\
    ~                                       & ~                          & SP ($\times 10^{5}$) & 0.56±.08 & 0.11±.01 & 0.59±.08 & 0.11±.01 & 0.10±.01 \\
    \cmidrule[\heavyrulewidth]{1-8}
    \multirow{27}*{\rotatebox{90}{Expert}}  & \multirow{3}*{Ant}         & HV ($\times 10^{6}$) & 5.88±.02 & 6.38±.01 & 4.76±.05 & 6.39±.02 & \textbf{6.40±.01} \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & 2.13±.02 & \textbf{2.15±.01} & 1.94±.02 & \textbf{2.15±.01} & \textbf{2.15±.01} \\
    ~                                       & ~                          & SP ($\times 10^{4}$) & 2.22±.50 & 0.75±.13 & 5.16±1.18 & 0.82±.25 & 0.71±.20 \\
    \cmidrule{2-8}
    ~                                       & \multirow{3}*{HalfCheetah} & HV ($\times 10^{6}$) & 5.69±.00 & 5.73±.00 & 5.66±.00 & \textbf{5.78±.00} & 5.77±.00 \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & \textbf{2.16±.00} & 2.13±.00 & 2.07±.01 & 2.09±.00 & 2.11±.00 \\
    ~                                       & ~                          & SP ($\times 10^{4}$) & 0.18±.01 & 0.15±.02 & 0.34±.03 & 0.10±.01 & 0.13±.01 \\
    \cmidrule{2-8}
    ~                                       & \multirow{3}*{Hopper}      & HV ($\times 10^{7}$) & 1.95±.03 & \textbf{2.07±.01} & 1.49±.01 & \textbf{2.07±.00} & \textbf{2.07±.00} \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & 4.02±.02 & \textbf{4.15±.03} & 3.66±.07 & 4.06±.01 & 4.05±.01 \\
    ~                                       & ~                          & SP ($\times 10^{5}$) & 0.85±.27 & 0.20±.06 & 2.58±1.01 & 0.11±.00 & 0.11±.02 \\
    \cmidrule{2-8}
    ~                                       & \multirow{3}*{Swimmer}     & HV ($\times 10^{4}$) & 3.20±.00 & \textbf{3.24±.00} & 3.19±.00 & \textbf{3.24±.00} & \textbf{3.24±.00} \\
    ~                                       & ~                          & WR ($\times 10^{2}$) & 1.56±.01 & \textbf{1.70±.01} & \textbf{1.70±.01} & 1.63±.01 & 1.64±.01 \\
    ~                                       & ~                          & SP ($\times 10^{0}$) & 15.50±.33 & 7.36±.81 & 9.05±.30 & 6.04±.48 & 9.03±1.08 \\
    \cmidrule{2-8}
    ~                                       & \multirow{3}*{Walker2d}    & HV ($\times 10^{6}$) & 5.01±.01 & 5.14±.01 & 3.47±.12 & \textbf{5.20±.00} & \textbf{5.20±.00} \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & \textbf{2.04±.00} & 1.98±.01 & 1.45±.04 & 1.96±.00 & 1.97±.00 \\
    ~                                       & ~                          & SP ($\times 10^{4}$) & 0.49±.03 & 0.27±.04 & 16.61±13.78 & 0.12±.00 & 0.14±.01 \\
    \cmidrule{2-8}
    ~                                       & \multirow{3}*{Hopper-3obj} & HV ($\times 10^{10}$) & 2.83±.06 & 3.28±.07 & 1.95±.16 & 3.36±.03 & \textbf{3.39±.04} \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & 2.16±.02 & \textbf{2.46±.00} & 1.96±.05 & 2.29±.01 & 2.27±.04 \\
    ~                                       & ~                          & SP ($\times 10^{5}$) & 0.09±.01 & 0.06±.00 & 0.17±.06 & 0.11±.01 & 0.12±.01 \\

    \bottomrule
  \end{tabular}
\end{table*}

\begin{table*}[htb]
  \caption{Narrow}
  \label{sample-table}
  \centering
  \begin{tabular}{p{0.03\textwidth}p{0.1\textwidth}p{0.11\textwidth}||p{0.1\textwidth}p{0.1\textwidth}p{0.1\textwidth}|p{0.1\textwidth}p{0.1\textwidth}}
    \toprule
    ~ & \textbf{Env} & metrics & \textbf{MODT(P)} & \textbf{MORvS(P)} & \textbf{BC(P)} & \textbf{MODULI} & \textbf{MODULI w slider} \\
    \midrule
    \multirow{20}*{\rotatebox{90}{Amateur}} & \multirow{3}*{Ant}         & HV ($\times 10^{6}$) & 5.17±.03 & 5.80±.03 & 4.19±.10 & 5.85±.03 & \textbf{5.86±.02} \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & \textbf{2.07±.02} & \textbf{2.07±.01} & 1.76±.06 & 2.05±.00 & 2.06±.00 \\
    ~                                       & ~                          & SP ($\times 10^{4}$) & 0.43±.10 & 0.51±.08 & 4.42±1.44 & 0.62±.11 & 0.61±.09 \\
    \cmidrule{2-8}
    ~                                       & \multirow{3}*{HalfCheetah} & HV ($\times 10^{6}$) & 4.29±.00 & 5.55±.00 & 5.08±.01 & 5.72±.00 & \textbf{5.73±.00} \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & 2.15±.04 & 2.10±.00 & 2.12±.00 & 2.10±.00 & \textbf{2.17±.01} \\
    ~                                       & ~                          & SP ($\times 10^{4}$) & 1.02±.44 & 0.02±.00 & 0.02±.00 & 0.06±.00 & 0.05±.00 \\
    \cmidrule{2-8}
    ~                                       & \multirow{3}*{Hopper}      & HV ($\times 10^{7}$) & 1.73±.01 & 1.69±.01 & 0.94±.34 & 1.99±.01 & \textbf{2.01±.01} \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & 3.84±.01 & 3.90±.02 & 3.01±.58 & 3.96±.06 & \textbf{3.99±.01} \\
    ~                                       & ~                          & SP ($\times 10^{5}$) & 0.27±.07 & 0.15±.03 & 5.81±8.21 & 0.37±.18 & 0.18±.02 \\
    \cmidrule{2-8}
    ~                                       & \multirow{3}*{Swimmer}     & HV ($\times 10^{4}$) & 0.66±.03 & 2.95±.00 & 2.80±.00 & 3.14±.00 & \textbf{3.16±.00} \\
    ~                                       & ~                          & WR ($\times 10^{2}$) & 1.37±.05 & 1.48±.00 & 1.39±.00 & 1.59±.01 & \textbf{1.63±.01} \\
    ~                                       & ~                          & SP ($\times 10^{0}$) & 14.25±3.73 & 1.91±.01 & 2.95±.08 & 11.56±1.28 & 10.54±1.45 \\
    \cmidrule{2-8}
    ~                                       & \multirow{3}*{Walker2d}    & HV ($\times 10^{6}$) & 3.42±.16 & 4.83±.00 & 2.83±.01 & 4.91±.01 & \textbf{4.93±.00} \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & 1.75±.01 & 1.92±.00 & 1.76±.00 & 1.92±.00 & \textbf{1.94±.00} \\
    ~                                       & ~                          & SP ($\times 10^{4}$) & 5.64±3.72 & 0.22±.01 & 0.01±.00 & 0.24±.01 & 0.25±.01 \\
    \cmidrule{2-8}
    ~                                       & \multirow{3}*{Hopper-3obj} & HV ($\times 10^{10}$) & 1.85±.04 & 2.27±.05 & 2.26±.02 & 2.85±.06 & \textbf{2.96±.08} \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & \textbf{2.52±.03} & 2.15±.01 & 2.03±.01 & 2.11±.01 & 2.12±.02 \\
    ~                                       & ~                          & SP ($\times 10^{5}$) & 3.12±1.21 & 0.07±.01 & 0.09±.00 & 0.13±.01 & 0.12±.02 \\
    \cmidrule[\heavyrulewidth]{1-8}
    \multirow{27}*{\rotatebox{90}{Expert}}  & \multirow{3}*{Ant}         & HV ($\times 10^{6}$) & 5.05±.08 & 6.06±.00 & 4.90±.02 & \textbf{6.35±.01} & 6.31±.02 \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & 2.06±.02 & 2.11±.01 & 1.94±.02 & 2.19±.02 & \textbf{2.21±.03} \\
    ~                                       & ~                          & SP ($\times 10^{4}$) & 0.88±.41 & 0.79±.11 & 1.56±.28 & 0.73±.07 & 0.68±.16 \\
    \cmidrule{2-8}
    ~                                       & \multirow{3}*{HalfCheetah} & HV ($\times 10^{6}$) & 5.04±.00 & 5.46±.01 & 4.88±.02 & \textbf{5.76±.00} & \textbf{5.76±.00} \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & \textbf{2.16±.00} & 2.07±.00 & 2.13±.00 & 2.13±.01 & 2.13±.00 \\
    ~                                       & ~                          & SP ($\times 10^{4}$) & 0.04±.00 & 0.05±.00 & 0.02±.00 & 0.04±.00 & 0.04±.00 \\
    \cmidrule{2-8}
    ~                                       & \multirow{3}*{Hopper}      & HV ($\times 10^{7}$) & 1.85±.02 & 1.98±.00 & 1.29±.01 & \textbf{2.03±.01} & 2.02±.00 \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & \textbf{4.22±.02} & 4.09±.03 & 3.39±.02 & 4.06±.03 & 3.99±.00 \\
    ~                                       & ~                          & SP ($\times 10^{5}$) & 0.34±.07 & 0.16±.02 & 0.59±.24 & 0.30±.12 & 0.25±.04 \\
    \cmidrule{2-8}
    ~                                       & \multirow{3}*{Swimmer}     & HV ($\times 10^{4}$) & 3.03±.00 & 3.10±.00 & 3.06±.00 & \textbf{3.21±.00} & \textbf{3.21±.00} \\
    ~                                       & ~                          & WR ($\times 10^{2}$) & 1.52±.01 & 1.51±.01 & 1.50±.01 & 1.55±.01 & \textbf{1.63±.01} \\
    ~                                       & ~                          & SP ($\times 10^{0}$) & 3.65±.22 & 4.38±.80 & 5.53±.20 & 3.24±.13 & 2.93±.10 \\
    \cmidrule{2-8}
    ~                                       & \multirow{3}*{Walker2d}    & HV ($\times 10^{6}$) & 4.75±.01 & 4.85±.01 & 1.88±.95 & \textbf{5.10±.01} & 5.07±.01 \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & 1.90±.01 & 1.94±.00 & 0.92±.26 & 1.96±.00 & \textbf{1.99±.00} \\
    ~                                       & ~                          & SP ($\times 10^{4}$) & 0.34±.09 & 0.19±.02 & 10.76±11.58 & 0.15±.04 & 0.13±.01 \\
    \cmidrule{2-8}
    ~                                       & \multirow{3}*{Hopper-3obj} & HV ($\times 10^{10}$) & 3.18±.05 & 3.32±.00 & 2.32±.10 & 3.33±.04 & \textbf{3.34±.05} \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & 2.30±.03 & \textbf{2.44±.02} & 2.01±.01 & 2.29±.03 & 2.23±.02 \\
    ~                                       & ~                          & SP ($\times 10^{5}$) & 0.11±.01 & 0.22±.02 & 0.14±.02 & 0.14±.02 & 0.12±.01 \\

    \bottomrule
  \end{tabular}
\end{table*}

==> tables/shattered_new_wr_full.tex <==
\begin{table*}[htb]
  \caption{new wr results on \texttt{Shattered} datasets.}
  \label{sample-table}
  \centering
  \begin{tabular}{p{0.03\textwidth}p{0.1\textwidth}p{0.11\textwidth}||p{0.1\textwidth}p{0.1\textwidth}p{0.1\textwidth}|p{0.1\textwidth}p{0.1\textwidth}}
    \toprule
    ~ & \textbf{Env} & metrics & \textbf{MODT(P)} & \textbf{MORvS(P)} & \textbf{BC(P)} & \textbf{MODULI} & \textbf{MODULI w slider} \\
    \midrule
    \multirow{27}*{\rotatebox{90}{Amateur}} & \multirow{3}*{Ant}         & HV ($\times 10^{6}$) & 5.74±.04 & \textbf{6.09±.01} & 4.20±.05 & 5.85±.03 & 5.86±.02 \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & 0.36±.01 & 0.13±.03 & 1.01±.07 & \textbf{0.10±.00} & \textbf{0.10±.00} \\
    ~                                       & ~                          & SP ($\times 10^{4}$) & 2.47±.61 & 0.79±.14 & 2.29±1.38 & 0.62±.11 & 0.61±.09 \\
    \cmidrule{2-8}
    ~                                       & \multirow{3}*{HalfCheetah} & HV ($\times 10^{6}$) & 5.61±.01 & \textbf{5.74±.00} & 5.54±.00 & 5.72±.00 & 5.73±.00 \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & 0.62±.00 & \textbf{0.10±.00} & 0.11±.00 & 0.18±.05 & 0.18±.02 \\
    ~                                       & ~                          & SP ($\times 10^{4}$) & 0.11±.01 & 0.09±.01 & 0.09±.01 & 0.06±.00 & 0.05±.00 \\
    \cmidrule{2-8}
    ~                                       & \multirow{3}*{Hopper}      & HV ($\times 10^{7}$) & 1.46±.00 & 1.69±.01 & 1.63±.00 & 1.99±.01 & \textbf{2.01±.01} \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & 2.51±.01 & 1.76±.02 & 0.99±.06 & \textbf{0.42±.06} & 0.49±.14 \\
    ~                                       & ~                          & SP ($\times 10^{5}$) & 0.54±.58 & 0.08±.01 & 0.11±.05 & 0.37±.18 & 0.18±.02 \\
    \cmidrule{2-8}
    ~                                       & \multirow{3}*{Swimmer}     & HV ($\times 10^{4}$) & 0.75±.00 & 2.81±.00 & 2.81±.00 & 3.14±.00 & \textbf{3.16±.00} \\
    ~                                       & ~                          & WR ($\times 10^{2}$) & 0.94±.00 & 0.40±.00 & 0.35±.00 & \textbf{0.34±.00} & \textbf{0.34±.00} \\
    ~                                       & ~                          & SP ($\times 10^{0}$) & 6.75±.23 & 1.26±.06 & 1.89±.05 & 11.56±1.28 & 10.54±1.45 \\
    \cmidrule{2-8}
    ~                                       & \multirow{3}*{Walker2d}    & HV ($\times 10^{6}$) & 3.86±.07 & \textbf{4.99±.00} & 3.42±.02 & 4.91±.01 & 4.93±.00 \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & 1.44±.02 & 0.23±.00 & 1.18±.01 & \textbf{0.06±.01} & 0.07±.02 \\
    ~                                       & ~                          & SP ($\times 10^{4}$) & 11.13±3.58 & 0.20±.03 & 4.56±.08 & 0.24±.01 & 0.25±.01 \\
    \cmidrule{2-8}
    ~                                       & \multirow{3}*{Hopper-3obj} & HV ($\times 10^{10}$) & 1.48±.02 & 2.84±.04 & 1.34±.02 & 2.85±.06 & \textbf{2.96±.08} \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & 2.86±.01 & \textbf{1.29±.01} & 2.87±.00 & 1.50±.07 & 1.50±.02 \\
    ~                                       & ~                          & SP ($\times 10^{5}$) & 0.56±.08 & 0.11±.01 & 0.59±.08 & 0.13±.01 & 0.12±.02 \\
    \cmidrule[\heavyrulewidth]{1-8}
    \multirow{27}*{\rotatebox{90}{Expert}}  & \multirow{3}*{Ant}         & HV ($\times 10^{6}$) & 5.88±.02 & \textbf{6.38±.01} & 4.76±.05 & 6.35±.01 & 6.31±.02 \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & 0.71±.03 & \textbf{0.16±.00} & 0.61±.01 & 0.19±.00 & 0.19±.00 \\
    ~                                       & ~                          & SP ($\times 10^{4}$) & 2.22±.50 & 0.75±.13 & 5.16±1.18 & 0.73±.07 & 0.68±.16 \\
    \cmidrule{2-8}
    ~                                       & \multirow{3}*{HalfCheetah} & HV ($\times 10^{6}$) & 5.69±.00 & 5.73±.00 & 5.66±.00 & \textbf{5.76±.00} & \textbf{5.76±.00} \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & 0.18±.00 & 0.10±.00 & 0.28±.00 & \textbf{0.04±.00} & \textbf{0.04±.00} \\
    ~                                       & ~                          & SP ($\times 10^{4}$) & 0.18±.01 & 0.15±.02 & 0.34±.03 & 0.04±.00 & 0.04±.00 \\
    \cmidrule{2-8}
    ~                                       & \multirow{3}*{Hopper}      & HV ($\times 10^{7}$) & 1.95±.03 & \textbf{2.07±.01} & 1.49±.01 & 2.03±.01 & 2.02±.00 \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & 1.42±.00 & 1.10±.04 & 3.92±.11 & 0.84±.15 & \textbf{0.78±.09} \\
    ~                                       & ~                          & SP ($\times 10^{5}$) & 0.85±.27 & 0.20±.06 & 2.58±1.01 & 0.30±.12 & 0.25±.04 \\
    \cmidrule{2-8}
    ~                                       & \multirow{3}*{Swimmer}     & HV ($\times 10^{4}$) & 3.20±.00 & \textbf{3.24±.00} & 3.19±.00 & 3.21±.00 & 3.21±.00 \\
    ~                                       & ~                          & WR ($\times 10^{2}$) & 0.38±.00 & 0.16±.00 & 0.07±.00 & \textbf{0.02±.00} & \textbf{0.02±.00} \\
    ~                                       & ~                          & SP ($\times 10^{0}$) & 15.50±.33 & 7.36±.81 & 9.05±.30 & 3.24±.13 & 2.93±.10 \\
    \cmidrule{2-8}
    ~                                       & \multirow{3}*{Walker2d}    & HV ($\times 10^{6}$) & 5.01±.01 & \textbf{5.14±.01} & 3.47±.12 & 5.10±.01 & 5.07±.01 \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & 0.86±.01 & 0.65±.02 & 1.72±.01 & 0.21±.05 & \textbf{0.19±.01} \\
    ~                                       & ~                          & SP ($\times 10^{4}$) & 0.49±.03 & 0.27±.04 & 16.61±13.78 & 0.15±.04 & 0.13±.01 \\
    \cmidrule{2-8}
    ~                                       & \multirow{3}*{Hopper-3obj} & HV ($\times 10^{10}$) & 2.83±.06 & 3.28±.07 & 1.95±.16 & 3.33±.04 & \textbf{3.34±.05} \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & \textbf{1.60±.01} & \textbf{1.60±.02} & 3.21±.01 & 1.76±.03 & 1.72±.08 \\
    ~                                       & ~                          & SP ($\times 10^{5}$) & 0.09±.01 & 0.06±.00 & 0.17±.06 & 0.14±.02 & 0.12±.01 \\

    \bottomrule
  \end{tabular}
\end{table*}

\begin{table*}[htb]
  \caption{new wr results on \texttt{Narrow} datasets.}
  \label{sample-table}
  \centering
  \begin{tabular}{p{0.03\textwidth}p{0.1\textwidth}p{0.11\textwidth}||p{0.1\textwidth}p{0.1\textwidth}p{0.1\textwidth}|p{0.1\textwidth}p{0.1\textwidth}}
    \toprule
    ~ & \textbf{Env} & metrics & \textbf{MODT(P)} & \textbf{MORvS(P)} & \textbf{BC(P)} & \textbf{MODULI} & \textbf{MODULI w slider} \\
    \midrule
    \multirow{27}*{\rotatebox{90}{Amateur}} & \multirow{3}*{Ant}         & HV ($\times 10^{6}$) & 5.17±.03 & 5.80±.03 & 4.19±.10 & 5.85±.03 & \textbf{5.86±.02} \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & 0.77±.01 & 0.27±.02 & 1.93±.04 & 0.55±.01 & \textbf{0.21±.04} \\
    ~                                       & ~                          & SP ($\times 10^{4}$) & 0.43±.10 & 0.51±.08 & 4.42±1.44 & 0.62±.11 & 0.61±.09 \\
    \cmidrule{2-8}
    ~                                       & \multirow{3}*{HalfCheetah} & HV ($\times 10^{6}$) & 4.29±.00 & 5.55±.00 & 5.08±.01 & 5.72±.00 & \textbf{5.73±.00} \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & 0.98±.01 & 0.33±.00 & 0.36±.00 & 0.46±.01 & \textbf{0.29±.02} \\
    ~                                       & ~                          & SP ($\times 10^{4}$) & 1.02±.44 & 0.02±.00 & 0.02±.00 & 0.06±.00 & 0.05±.00 \\
    \cmidrule{2-8}
    ~                                       & \multirow{3}*{Hopper}      & HV ($\times 10^{7}$) & 1.73±.01 & 1.69±.01 & 0.94±.34 & 1.99±.01 & \textbf{2.01±.01} \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & 1.38±.04 & 2.88±.08 & 5.22±.01 & 1.05±.11 & \textbf{0.60±.09} \\
    ~                                       & ~                          & SP ($\times 10^{5}$) & 0.27±.07 & 0.15±.03 & 5.81±8.21 & 0.37±.18 & 0.18±.02 \\
    \cmidrule{2-8}
    ~                                       & \multirow{3}*{Swimmer}     & HV ($\times 10^{4}$) & 0.66±.03 & 2.95±.00 & 2.80±.00 & 3.14±.00 & \textbf{3.16±.00} \\
    ~                                       & ~                          & WR ($\times 10^{2}$) & 1.14±.00 & \textbf{0.48±.00} & 0.49±.00 & 0.56±.00 & 0.55±.00 \\
    ~                                       & ~                          & SP ($\times 10^{0}$) & 14.25±3.73 & 1.91±.01 & 2.95±.08 & 11.56±1.28 & 10.54±1.45 \\
    \cmidrule{2-8}
    ~                                       & \multirow{3}*{Walker2d}    & HV ($\times 10^{6}$) & 3.42±.16 & 4.83±.00 & 2.83±.01 & 4.91±.01 & \textbf{4.93±.00} \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & 1.91±.00 & 1.77±.00 & 1.87±.00 & 1.02±.01 & \textbf{0.82±.02} \\
    ~                                       & ~                          & SP ($\times 10^{4}$) & 5.64±3.72 & 0.22±.01 & 0.01±.00 & 0.24±.01 & 0.25±.01 \\
    \cmidrule{2-8}
    ~                                       & \multirow{3}*{Hopper-3obj} & HV ($\times 10^{10}$) & 1.85±.04 & 2.27±.05 & 2.26±.02 & 2.85±.06 & \textbf{2.96±.08} \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & 2.44±.02 & \textbf{1.59±.02} & 1.86±.03 & 2.26±.03 & 2.03±.02 \\
    ~                                       & ~                          & SP ($\times 10^{5}$) & 3.12±1.21 & 0.07±.01 & 0.09±.00 & 0.13±.01 & 0.12±.02 \\
    \cmidrule[\heavyrulewidth]{1-8}
    \multirow{27}*{\rotatebox{90}{Expert}}  & \multirow{3}*{Ant}         & HV ($\times 10^{6}$) & 5.05±.08 & 6.06±.00 & 4.90±.02 & \textbf{6.35±.01} & 6.31±.02 \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & 0.98±.01 & 0.37±.03 & 0.78±.03 & \textbf{0.23±.01} & 0.26±.00 \\
    ~                                       & ~                          & SP ($\times 10^{4}$) & 0.88±.41 & 0.79±.11 & 1.56±.28 & 0.73±.07 & 0.68±.16 \\
    \cmidrule{2-8}
    ~                                       & \multirow{3}*{HalfCheetah} & HV ($\times 10^{6}$) & 5.04±.00 & 5.46±.01 & 4.88±.02 & \textbf{5.76±.00} & \textbf{5.76±.00} \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & 0.43±.00 & 0.29±.00 & 0.44±.00 & \textbf{0.17±.00} & 0.18±.00 \\
    ~                                       & ~                          & SP ($\times 10^{4}$) & 0.04±.00 & 0.05±.00 & 0.02±.00 & 0.04±.00 & 0.04±.00 \\
    \cmidrule{2-8}
    ~                                       & \multirow{3}*{Hopper}      & HV ($\times 10^{7}$) & 1.85±.02 & 1.98±.00 & 1.29±.01 & \textbf{2.03±.01} & 2.02±.00 \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & 4.24±.02 & 1.37±.05 & 3.83±.05 & 2.62±.05 & \textbf{0.80±.08} \\
    ~                                       & ~                          & SP ($\times 10^{5}$) & 0.34±.07 & 0.16±.02 & 0.59±.24 & 0.30±.12 & 0.25±.04 \\
    \cmidrule{2-8}
    ~                                       & \multirow{3}*{Swimmer}     & HV ($\times 10^{4}$) & 3.03±.00 & 3.10±.00 & 3.06±.00 & \textbf{3.21±.00} & \textbf{3.21±.00} \\
    ~                                       & ~                          & WR ($\times 10^{2}$) & 0.38±.00 & 0.39±.01 & 0.19±.00 & \textbf{0.10±.00} & 0.13±.00 \\
    ~                                       & ~                          & SP ($\times 10^{0}$) & 3.65±.22 & 4.38±.80 & 5.53±.20 & 3.24±.13 & 2.93±.10 \\
    \cmidrule{2-8}
    ~                                       & \multirow{3}*{Walker2d}    & HV ($\times 10^{6}$) & 4.75±.01 & 4.85±.01 & 1.88±.95 & \textbf{5.10±.01} & 5.07±.01 \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & 1.07±.01 & 1.45±.02 & 1.88±.00 & 0.42±.02 & \textbf{0.21±.00} \\
    ~                                       & ~                          & SP ($\times 10^{4}$) & 0.34±.09 & 0.19±.02 & 10.76±11.58 & 0.15±.04 & 0.13±.01 \\
    \cmidrule{2-8}
    ~                                       & \multirow{3}*{Hopper-3obj} & HV ($\times 10^{10}$) & 3.18±.05 & 3.32±.00 & 2.32±.10 & 3.33±.04 & \textbf{3.34±.05} \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & 2.48±.00 & \textbf{2.24±.02} & 2.49±.02 & 2.62±.03 & 2.27±.05 \\
    ~                                       & ~                          & SP ($\times 10^{5}$) & 0.11±.01 & 0.22±.02 & 0.14±.02 & 0.14±.02 & 0.12±.01 \\

    \bottomrule
  \end{tabular}
\end{table*}

\begin{table*}[htb]
  \caption{new wr results on \texttt{Shattered} datasets. New implement.}
  \label{sample-table}
  \centering
  \begin{tabular}{p{0.03\textwidth}p{0.1\textwidth}p{0.11\textwidth}||p{0.1\textwidth}p{0.1\textwidth}p{0.1\textwidth}|p{0.1\textwidth}p{0.1\textwidth}}
    \toprule
    ~ & \textbf{Env} & metrics & \textbf{MODT(P)} & \textbf{MORvS(P)} & \textbf{BC(P)} & \textbf{MODULI} & \textbf{MODULI w slider} \\
    \midrule
    \multirow{27}*{\rotatebox{90}{Amateur}} & \multirow{3}*{Ant}         & HV ($\times 10^{6}$) & 5.74±.04 & \textbf{6.09±.01} & 4.20±.05 & 5.85±.03 & 5.88±.03 \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & 0.36±.01 & 0.13±.03 & 1.01±.07 & \textbf{0.10±.00} & 0.11±.01 \\
    ~                                       & ~                          & SP ($\times 10^{4}$) & 2.47±.61 & 0.79±.14 & 2.29±1.38 & 0.62±.11 & 0.92±.08 \\
    \cmidrule{2-8}
    ~                                       & \multirow{3}*{HalfCheetah} & HV ($\times 10^{6}$) & 5.61±.01 & \textbf{5.74±.00} & 5.54±.00 & 5.72±.00 & 5.71±.00 \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & 0.62±.00 & \textbf{0.10±.00} & 0.11±.00 & 0.18±.05 & 0.17±.02 \\
    ~                                       & ~                          & SP ($\times 10^{4}$) & 0.11±.01 & 0.09±.01 & 0.09±.01 & 0.06±.00 & 0.06±.00 \\
    \cmidrule{2-8}
    ~                                       & \multirow{3}*{Hopper}      & HV ($\times 10^{7}$) & 1.46±.00 & 1.69±.01 & 1.63±.00 & \textbf{1.99±.01} & \textbf{1.99±.00} \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & 2.51±.01 & 1.76±.02 & 0.99±.06 & 0.42±.06 & \textbf{0.39±.06} \\
    ~                                       & ~                          & SP ($\times 10^{5}$) & 0.54±.58 & 0.08±.01 & 0.11±.05 & 0.37±.18 & 0.26±.06 \\
    \cmidrule{2-8}
    ~                                       & \multirow{3}*{Swimmer}     & HV ($\times 10^{4}$) & 0.75±.00 & 2.81±.00 & 2.81±.00 & 3.14±.00 & \textbf{3.15±.00} \\
    ~                                       & ~                          & WR ($\times 10^{2}$) & 0.94±.00 & 0.40±.00 & 0.35±.00 & \textbf{0.34±.00} & \textbf{0.34±.00} \\
    ~                                       & ~                          & SP ($\times 10^{0}$) & 6.75±.23 & 1.26±.06 & 1.89±.05 & 11.56±1.28 & 11.58±1.75 \\
    \cmidrule{2-8}
    ~                                       & \multirow{3}*{Walker2d}    & HV ($\times 10^{6}$) & 3.86±.07 & \textbf{4.99±.00} & 3.42±.02 & 4.91±.01 & 4.91±.01 \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & 1.44±.02 & 0.23±.00 & 1.18±.01 & \textbf{0.06±.01} & 0.07±.00 \\
    ~                                       & ~                          & SP ($\times 10^{4}$) & 11.13±3.58 & 0.20±.03 & 4.56±.08 & 0.24±.01 & 0.26±.03 \\
    \cmidrule{2-8}
    ~                                       & \multirow{3}*{Hopper-3obj} & HV ($\times 10^{10}$) & 1.48±.02 & 2.84±.04 & 1.34±.02 & \textbf{2.85±.06} & - \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & 2.86±.01 & \textbf{1.29±.01} & 2.87±.00 & 1.50±.07 & - \\
    ~                                       & ~                          & SP ($\times 10^{5}$) & 0.56±.08 & 0.11±.01 & 0.59±.08 & 0.13±.01 & - \\
    \cmidrule[\heavyrulewidth]{1-8}
    \multirow{27}*{\rotatebox{90}{Expert}}  & \multirow{3}*{Ant}         & HV ($\times 10^{6}$) & 5.88±.02 & \textbf{6.38±.01} & 4.76±.05 & 6.35±.01 & 6.36±.00 \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & 0.71±.03 & \textbf{0.16±.00} & 0.61±.01 & 0.19±.00 & 0.20±.00 \\
    ~                                       & ~                          & SP ($\times 10^{4}$) & 2.22±.50 & 0.75±.13 & 5.16±1.18 & 0.73±.07 & 0.81±.25 \\
    \cmidrule{2-8}
    ~                                       & \multirow{3}*{HalfCheetah} & HV ($\times 10^{6}$) & 5.69±.00 & 5.73±.00 & 5.66±.00 & \textbf{5.76±.00} & \textbf{5.76±.00} \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & 0.18±.00 & 0.10±.00 & 0.28±.00 & \textbf{0.04±.00} & \textbf{0.04±.00} \\
    ~                                       & ~                          & SP ($\times 10^{4}$) & 0.18±.01 & 0.15±.02 & 0.34±.03 & 0.04±.00 & 0.04±.00 \\
    \cmidrule{2-8}
    ~                                       & \multirow{3}*{Hopper}      & HV ($\times 10^{7}$) & 1.95±.03 & \textbf{2.07±.01} & 1.49±.01 & 2.03±.01 & 2.04±.01 \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & 1.42±.00 & 1.10±.04 & 3.92±.11 & 0.84±.15 & \textbf{0.77±.06} \\
    ~                                       & ~                          & SP ($\times 10^{5}$) & 0.85±.27 & 0.20±.06 & 2.58±1.01 & 0.30±.12 & 0.25±.05 \\
    \cmidrule{2-8}
    ~                                       & \multirow{3}*{Swimmer}     & HV ($\times 10^{4}$) & 3.20±.00 & \textbf{3.24±.00} & 3.19±.00 & 3.21±.00 & 3.21±.00 \\
    ~                                       & ~                          & WR ($\times 10^{2}$) & 0.38±.00 & 0.16±.00 & 0.07±.00 & \textbf{0.02±.00} & \textbf{0.02±.00} \\
    ~                                       & ~                          & SP ($\times 10^{0}$) & 15.50±.33 & 7.36±.81 & 9.05±.30 & 3.24±.13 & 3.28±.15 \\
    \cmidrule{2-8}
    ~                                       & \multirow{3}*{Walker2d}    & HV ($\times 10^{6}$) & 5.01±.01 & \textbf{5.14±.01} & 3.47±.12 & 5.10±.01 & 5.10±.01 \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & 0.86±.01 & 0.65±.02 & 1.72±.01 & 0.21±.05 & \textbf{0.16±.02} \\
    ~                                       & ~                          & SP ($\times 10^{4}$) & 0.49±.03 & 0.27±.04 & 16.61±13.78 & 0.15±.04 & 0.13±.01 \\
    \cmidrule{2-8}
    ~                                       & \multirow{3}*{Hopper-3obj} & HV ($\times 10^{10}$) & 2.83±.06 & 3.28±.07 & 1.95±.16 & \textbf{3.33±.04} & - \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & \textbf{1.60±.01} & \textbf{1.60±.02} & 3.21±.01 & 1.76±.03 & - \\
    ~                                       & ~                          & SP ($\times 10^{5}$) & 0.09±.01 & 0.06±.00 & 0.17±.06 & 0.14±.02 & - \\

    \bottomrule
  \end{tabular}
\end{table*}

\begin{table*}[htb]
  \caption{new wr results on \texttt{Narrow} datasets. new Implement.}
  \label{sample-table}
  \centering
  \begin{tabular}{p{0.03\textwidth}p{0.1\textwidth}p{0.11\textwidth}||p{0.1\textwidth}p{0.1\textwidth}p{0.1\textwidth}|p{0.1\textwidth}p{0.1\textwidth}}
    \toprule
    ~ & \textbf{Env} & metrics & \textbf{MODT(P)} & \textbf{MORvS(P)} & \textbf{BC(P)} & \textbf{MODULI} & \textbf{MODULI w slider} \\
    \midrule
    \multirow{27}*{\rotatebox{90}{Amateur}} & \multirow{3}*{Ant}         & HV ($\times 10^{6}$) & 5.17±.03 & 5.80±.03 & 4.19±.10 & 5.85±.03 & \textbf{5.88±.03} \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & 0.77±.01 & \textbf{0.27±.02} & 1.93±.04 & 0.55±.01 & 0.53±.00 \\
    ~                                       & ~                          & SP ($\times 10^{4}$) & 0.43±.10 & 0.51±.08 & 4.42±1.44 & 0.62±.11 & 0.92±.08 \\
    \cmidrule{2-8}
    ~                                       & \multirow{3}*{HalfCheetah} & HV ($\times 10^{6}$) & 4.29±.00 & 5.55±.00 & 5.08±.01 & \textbf{5.72±.00} & 5.71±.00 \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & 0.98±.01 & \textbf{0.33±.00} & 0.36±.00 & 0.46±.01 & 0.35±.01 \\
    ~                                       & ~                          & SP ($\times 10^{4}$) & 1.02±.44 & 0.02±.00 & 0.02±.00 & 0.06±.00 & 0.06±.00 \\
    \cmidrule{2-8}
    ~                                       & \multirow{3}*{Hopper}      & HV ($\times 10^{7}$) & 1.73±.01 & 1.69±.01 & 0.94±.34 & \textbf{1.99±.01} & \textbf{1.99±.00} \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & 1.38±.04 & 2.88±.08 & 5.22±.01 & \textbf{1.05±.11} & 1.33±.18 \\
    ~                                       & ~                          & SP ($\times 10^{5}$) & 0.27±.07 & 0.15±.03 & 5.81±8.21 & 0.37±.18 & 0.26±.06 \\
    \cmidrule{2-8}
    ~                                       & \multirow{3}*{Swimmer}     & HV ($\times 10^{4}$) & 0.66±.03 & 2.95±.00 & 2.80±.00 & 3.14±.00 & \textbf{3.15±.00} \\
    ~                                       & ~                          & WR ($\times 10^{2}$) & 1.14±.00 & \textbf{0.48±.00} & 0.49±.00 & 0.56±.00 & 0.55±.00 \\
    ~                                       & ~                          & SP ($\times 10^{0}$) & 14.25±3.73 & 1.91±.01 & 2.95±.08 & 11.56±1.28 & 11.58±1.75 \\
    \cmidrule{2-8}
    ~                                       & \multirow{3}*{Walker2d}    & HV ($\times 10^{6}$) & 3.42±.16 & 4.83±.00 & 2.83±.01 & \textbf{4.91±.01} & \textbf{4.91±.01} \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & 1.91±.00 & 1.77±.00 & 1.87±.00 & 1.02±.01 & \textbf{0.97±.02} \\
    ~                                       & ~                          & SP ($\times 10^{4}$) & 5.64±3.72 & 0.22±.01 & 0.01±.00 & 0.24±.01 & 0.26±.03 \\
    \cmidrule{2-8}
    ~                                       & \multirow{3}*{Hopper-3obj} & HV ($\times 10^{10}$) & 1.85±.04 & 2.27±.05 & 2.26±.02 & \textbf{2.85±.06} & - \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & 2.44±.02 & \textbf{1.59±.02} & 1.86±.03 & 2.26±.03 & - \\
    ~                                       & ~                          & SP ($\times 10^{5}$) & 3.12±1.21 & 0.07±.01 & 0.09±.00 & 0.13±.01 & - \\
    \cmidrule[\heavyrulewidth]{1-8}
    \multirow{27}*{\rotatebox{90}{Expert}}  & \multirow{3}*{Ant}         & HV ($\times 10^{6}$) & 5.05±.08 & 6.06±.00 & 4.90±.02 & 6.35±.01 & \textbf{6.36±.00} \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & 0.98±.01 & 0.37±.03 & 0.78±.03 & \textbf{0.23±.01} & 0.25±.01 \\
    ~                                       & ~                          & SP ($\times 10^{4}$) & 0.88±.41 & 0.79±.11 & 1.56±.28 & 0.73±.07 & 0.81±.25 \\
    \cmidrule{2-8}
    ~                                       & \multirow{3}*{HalfCheetah} & HV ($\times 10^{6}$) & 5.04±.00 & 5.46±.01 & 4.88±.02 & \textbf{5.76±.00} & \textbf{5.76±.00} \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & 0.43±.00 & 0.29±.00 & 0.44±.00 & \textbf{0.17±.00} & \textbf{0.17±.00} \\
    ~                                       & ~                          & SP ($\times 10^{4}$) & 0.04±.00 & 0.05±.00 & 0.02±.00 & 0.04±.00 & 0.04±.00 \\
    \cmidrule{2-8}
    ~                                       & \multirow{3}*{Hopper}      & HV ($\times 10^{7}$) & 1.85±.02 & 1.98±.00 & 1.29±.01 & 2.03±.01 & \textbf{2.04±.01} \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & 4.24±.02 & \textbf{1.37±.05} & 3.83±.05 & 2.62±.05 & 2.42±.05 \\
    ~                                       & ~                          & SP ($\times 10^{5}$) & 0.34±.07 & 0.16±.02 & 0.59±.24 & 0.30±.12 & 0.25±.05 \\
    \cmidrule{2-8}
    ~                                       & \multirow{3}*{Swimmer}     & HV ($\times 10^{4}$) & 3.03±.00 & 3.10±.00 & 3.06±.00 & \textbf{3.21±.00} & \textbf{3.21±.00} \\
    ~                                       & ~                          & WR ($\times 10^{2}$) & 0.38±.00 & 0.39±.01 & 0.19±.00 & \textbf{0.10±.00} & \textbf{0.10±.00} \\
    ~                                       & ~                          & SP ($\times 10^{0}$) & 3.65±.22 & 4.38±.80 & 5.53±.20 & 3.24±.13 & 3.28±.15 \\
    \cmidrule{2-8}
    ~                                       & \multirow{3}*{Walker2d}    & HV ($\times 10^{6}$) & 4.75±.01 & 4.85±.01 & 1.88±.95 & \textbf{5.10±.01} & \textbf{5.10±.01} \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & 1.07±.01 & 1.45±.02 & 1.88±.00 & 0.42±.02 & \textbf{0.28±.02} \\
    ~                                       & ~                          & SP ($\times 10^{4}$) & 0.34±.09 & 0.19±.02 & 10.76±11.58 & 0.15±.04 & 0.13±.01 \\
    \cmidrule{2-8}
    ~                                       & \multirow{3}*{Hopper-3obj} & HV ($\times 10^{10}$) & 3.18±.05 & 3.32±.00 & 2.32±.10 & \textbf{3.33±.04} & - \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & 2.48±.00 & \textbf{2.24±.02} & 2.49±.02 & 2.62±.03 & - \\
    ~                                       & ~                          & SP ($\times 10^{5}$) & 0.11±.01 & 0.22±.02 & 0.14±.02 & 0.14±.02 & - \\

    \bottomrule
  \end{tabular}
\end{table*}

==> tables/shattered_partial.tex <==
\begin{table*}[htb]
  \caption{Results on \texttt{Shattered} and \texttt{Narrow} datasets.}
  \label{sample-table}
  \centering
  \begin{tabular}{p{0.03\textwidth}p{0.1\textwidth}p{0.11\textwidth}||p{0.1\textwidth}p{0.1\textwidth}p{0.1\textwidth}|p{0.1\textwidth}p{0.1\textwidth}}
    \toprule
    ~ & \textbf{Env} & metrics & \textbf{MODT(P)} & \textbf{MORvS(P)} & \textbf{BC(P)} & \textbf{MODULI} & \textbf{MODULI w slider} \\
    \midrule
    \multirow{6}*{\rotatebox{90}{Shattered}} & \multirow{3}*{Hopper}      & HV ($\times 10^{7}$) & 1.46±.00 & 1.69±.01 & 1.63±.00 & 2.00±.00 & \textbf{2.01±.00} \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & 3.90±.02 & 3.85±.02 & 3.70±.01 & 3.96±.00 & \textbf{4.00±.04} \\
    ~                                       & ~                          & SP ($\times 10^{5}$) & 0.54±.58 & 0.08±.01 & 0.11±.05 & 0.17±.02 & 0.19±.01 \\
    \cmidrule{2-8}
    ~                                       & \multirow{3}*{Swimmer}     & HV ($\times 10^{4}$) & 0.75±.00 & 2.81±.00 & 2.81±.00 & \textbf{3.18±.01} & \textbf{3.18±.00} \\
    ~                                       & ~                          & WR ($\times 10^{2}$) & 1.38±.00 & 1.43±.00 & 1.48±.00 & 1.62±.02 & \textbf{1.65±.02} \\
    ~                                       & ~                          & SP ($\times 10^{0}$) & 6.75±.23 & 1.26±.06 & 1.89±.05 & 8.85±.77 & 15.71±.61 \\
    \cmidrule[\heavyrulewidth]{1-8}
    \multirow{6}*{\rotatebox{90}{Narrow}}  & \multirow{3}*{Hopper}      & HV ($\times 10^{7}$) & 1.73±.01 & 1.69±.01 & 0.94±.34 & 1.99±.01 & \textbf{2.01±.01} \\
    ~                                       & ~                          & WR ($\times 10^{3}$) & 3.84±.01 & 3.90±.02 & 3.01±.58 & 3.96±.06 & \textbf{3.99±.01} \\
    ~                                       & ~                          & SP ($\times 10^{5}$) & 0.27±.07 & 0.15±.03 & 5.81±8.21 & 0.37±.18 & 0.18±.02 \\
    \cmidrule{2-8}
    ~                                       & \multirow{3}*{Swimmer}     & HV ($\times 10^{4}$) & 0.66±.03 & 2.95±.00 & 2.80±.00 & 3.14±.00 & \textbf{3.16±.00} \\
    ~                                       & ~                          & WR ($\times 10^{2}$) & 1.37±.05 & 1.48±.00 & 1.39±.00 & 1.59±.01 & \textbf{1.63±.01} \\
    ~                                       & ~                          & SP ($\times 10^{0}$) & 14.25±3.73 & 1.91±.01 & 2.95±.08 & 11.56±1.28 & 10.54±1.45 \\
    \bottomrule
  \end{tabular}
\end{table*}
